Optimal Congestion Control for Time-varying Wireless Links

Modern networks exhibit a high degree of variability in link rates. Cellular network bandwidth inherently varies with receiver motion and orientation, while class-based packet scheduling in datacenter and service provider networks induces high variability in available capacity for network tenants. Recent work has proposed numerous congestion control protocols to cope with this variability, offering different tradeoffs between link utilization and queuing delay. In this paper, we develop a formal model of congestion control over time-varying links, and we use this model to derive a bound on the performance of any congestion control protocol running over a time-varying link with a given distribution of rate variation. Using the insights from this analysis, we derive an optimal control law that offers a smooth tradeoff between link utilization and queuing delay. We compare the performance of this control law to several existing control algorithms on cellular link traces to show that there is significant room for optimization.

==> SIGMETRICS/Model1.tex <==
\section{A Simple Link Model}
\label{s:model1}
%\subsection{Model}
\label{ss:model1:model}
%We consider a network with a single sender and receiver pair connected via a time-varying link. We consider a discrete time model, where each discrete round's duration is $T$, the base RTT for the sender-receiver pair.
We begin with a simple model where $\mu(t)$ deviates from $\mu(t-1)$ by an I.I.D. multiplicative factor. We refer to this as the Multiplicative I.I.D. Factors (MIF) model. Our analysis of the MIF model forms the basis for studying more complex link models later in the paper. 

Formally, $\mu(t)$ evolves according to: 
\begin{equation}
    \mu(t) = \mu(t - 1) \cdot X_t,
    \label{eq:model1:model}
\end{equation}
where $X_t$ is a I.I.D random variable with probability density function (PDF) $f(\cdot)$. Since we don't want the link capacity to drop below zero, we assume that $X_t$ is positive. 
%\ma{The link capacity evolution is independent of the state of the link and the sending rate decisions of the congestion control algorithm, i.e. $X_t$ is independent of $Q(t-1)$, $\mu(t-1)$ and $s(t)$.} 
The link capacity evolution is independent of the sending rate decisions of the congestion control algorithm, formally, $X_t$ is independent of $Q(i)$, $\mu(i)$ and $s(i), \forall i < t$. Additionally, independence of $s(t)$ and $X_t$ follows from the assumption that the congestion control algorithm is causal and does not have advanced knowledge of future capacity variations (although it is permitted to know the {\em distribution} of the variations). %\pg{Check this.}


%Also we assume there is some distribution on the starting link rate ($\mu(0)$), and $\mu(0)>0$. 

%We also assume that in round 1, $\mu(0)$ is known. 

We will first establish a performance bound in terms of the expected underutilization ($E[\bar{U}(t)]$) and expected queuing delay ($E[\bar{q}(t)]$) that can be achieved by {\em any} causal congestion control algorithm. We use this analysis to draw insights about the optimal congestion controller for this setting (\S\ref{ss:model1:achievable_bound}). Finally, we will derive the exact optimal control law by posing the problem of deciding the sending rate as a Markov Decision Process (MDP) (\S\ref{ss:model1:mdp}). In \S\ref{ss:model1:implications}, we will discuss the implications of our analysis and validate our findings using real-world cellular traces.
%We will also draw insights about the optimal congestion control law for causal protocols.

\subsection{Performance Bound}
\label{ss:model1:performance_bound}

\begin{theorem} 
In the MIF model, for any causal congestion control protocol and any $t \in \mathbb{N}$, the point $(E[\bar{q}(t)]$, $E[\bar{U}(t)])$ always lies in a convex set $\mathbb{C}^f \triangleq \{(x,y) | y \geq g^f(x)\}$, where $g^f(\cdot)$ is defined as follows:
\begin{align}
    x &= T \cdot \int_{0}^{b}\left(\frac{b}{a} - 1 \right) \cdot f(a) \cdot da, & g^f(x) &= \int_{b}^{\infty}\left( 1 - \frac{b}{a}\right) \cdot f(a) \cdot da, 
\label{eq:model1:thm:perfbound}
\end{align}
where $b \in \mathbb{R}^+$.
\label{thm:model1:perfbound}
\end{theorem}

\if 0
\begin{theorem} 
In the MIF model, for any causal congestion control protocol, and any $t \in \mathbb{N}$, there is a fundamental trade-off between $E[\bar{q}(t)]$ and $E[\bar{U}(t)]$. The point \{$E[\bar{q}(t)]$, $E[\bar{U}(t)]$\} always lies in a convex set $\mathbb{C}^f := \{\{x,y\} | y>=g^f(x)\}$. Where $g^f$ is defined as follows,
\begin{align}
    x &= T \cdot \int_{0}^{b}\left(\frac{b}{a} - 1 \right) \cdot f(a) \cdot da\nonumber\\
    g^f(x) &= \int_{b}^{\infty}\left( 1 - \frac{b}{a}\right) \cdot f(a) \cdot da 
\label{eq:model1:thm:perfbound}
\end{align}
where $b \in \mathbb{R}^+$.
\label{thm:model1:perfbound}
\end{theorem}
\fi

The curve $g^f(\cdot)$ forms the boundary of the set $\mathbb{C}^f$. Any causal congestion control strategy cannot achieve better performance in expectation than the feasible set $\mathbb{C}^f$. Note that in a particular run (i.e., for a given $\cup_{i=0}^{t}\{\mu(i)\}$), a scheme might get lucky and achieve performance $(\bar{q}(t), \bar{U}(t))$ that lies outside $\mathbb{C}^f$ (i.e. below $g^f(\cdot)$), however, in expectation the performance is bounded by $\mathbb{C}^f$. %\ma{I think we can drop the superscript $f$ from $C^f$ and $g^f$. It's implicit in the model and simple notation is better.}\pg{the f subscript is useful in model 3}

\if 0
\begin{wrapfigure}{r}{0.48\textwidth}
    %\centering
    \vspace{-2mm}
    \includegraphics[width=0.45\columnwidth]{images/feasible_uniform.pdf}
    \vspace{-4mm}
    \caption{\small {\bf Trade-off between underutilization and queuing delay, for $X \sim \textit{U}(0.27, 2) $, $T = 0.1$s ---} The gray region presents the feasible region of any congestion control protocol. The color of the performance bound ($g^f$) corresponds to different values of $b$ in Eq.~\eqref{eq:model1:thm:perfbound}.}
    \label{fig:model1:feasible_uniform}
    \vspace{-4.5mm}
\end{wrapfigure}

 
  \begin{figure}[t]
     \centering
    \includegraphics[width=0.6\columnwidth]{images/f_variation.pdf}
    \vspace{-4mm}
    \caption{\small {\bf Trade-off is dependent on the PDF $f$ ---} More variable the link is worse the performance bound.}
    \label{fig:model1:f_variation}
    \vspace{-4.5mm}
 \end{figure}
 \fi
 
 \begin{figure}[t]
\begin{minipage}[t]{.48\textwidth}
\centering
    \includegraphics[width=1\textwidth]{images/feasible_uniform.pdf}
    \vspace{-7mm}
    \caption{\small {\bf Trade-off between underutilization and queuing delay, for $X \sim \textit{U}(0.27, 2) $, $T = 0.1$s ---} The grey region presents that feasible region of any congestion control protocol. The color of the performance bound ($g^f(\cdot)$) corresponds to different value of $b$ in Eq.~\eqref{eq:model1:thm:perfbound}.}
    \label{fig:model1:feasible_uniform}
\end{minipage}
\hfill
\begin{minipage}[t]{.48\textwidth}
\centering
    \includegraphics[width=\textwidth]{images/f_variation.pdf}
    \vspace{-7mm}
    \caption{\small {\bf Trade-off is dependent on the PDF $f$ ---} The performance bound becomes worse (further up and to the right) as the extent of link rate variation increases.}
    \label{fig:model1:f_variation}
\end{minipage}
\vspace{-6mm}
\end{figure}
 
The performance bound depends on the distribution $f$ of the multiplicative factors $X_t$. \Fig{model1:feasible_uniform} shows this performance bound and the feasible region for a particular distribution. The distribution $f$ captures the {\em uncertainty} about the future link rate at each time step. If $X_t$ is highly variable, then the link rate $\mu(t)$ is highly uncertain (even with knowledge of $\mu(t-1)$). Our bound quantifies how this uncertainty imposes a limit on the achievable performance of any congestion control algorithm. For example, \Fig{model1:f_variation} shows the performance bound for two uniform distributions with different ranges. The more variable distribution imposes a worse bound on performance, shifting it upwards and to the right.% \ma{Can you use simple round numbers like U(0.3, 3) and U (0.5, 1.5) for the example. Something where it's immediately obvious what we mean by more variable.}

\subsubsection{Proof\\}
\label{ss:model1:proof_perfbound}
We first define a new quantity $\rho(t)$ in terms of $Q(t-1)$, $s(t)$ and $\mu(t-1)$ as follows,
\begin{align}
  \rho(t) =  \frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1)}.  
\label{eq:model1:proof_perfbound:rt}
\end{align}


In time step $t$, the total amount of data available (that can be serviced) at the link is $Q(t-1) + T \cdot s(t)$. Thus, $\rho(t)$ can be thought of as the ``load'' on the link in time step $t$ relative to the link capacity in previous time step $\mu(t-1)$.  With this new quantity, using $\mu(t) = \mu(t-1) \cdot X_t$, we can simplify Equations~\eqref{eq:setup:queue_delay_def} and ~\eqref{eq:setup:undeutilization_def} as follows: %\ma{use \eqref{} instead of \ref for equations}
\begin{align}
        q(t) &= \frac{(Q(t-1) + s(t) \cdot T - \mu(t) \cdot T)^+}{\mu(t)}= T \cdot \left(\frac{\rho(t)}{X_t} - 1 \right)^+,\nonumber\\
        U(t) &= \frac{(\mu(t) \cdot T - s(t) \cdot T - Q(t - 1))^+}{\mu(t) \cdot T} = \left(1 - \frac{\rho(t)}{X_t}\right)^+.
    \label{eq:model1:proof_perfbound:qU_rt}
    %\label{eq:model1:proof_perfbound:system}
\end{align}
Notice that both $q(t)$ and $U(t)$ depend only on $\rho(t)$ and the value of the random variable $X_{t}$. Moreover, $\rho(t)$ itself is a random variable dependent on $Q(t-1)$, $\mu(t-1)$, and the congestion control strategy (which selects $s(t)$). Crucially, $\rho(t)$ and $X_t$ are independent. We now use this independence to establish a bound on the expected underutuilization and queuing delay for a single time step $t$. But first, we need the following Lemma showing that the function $g^f$ is convex. 

%Notice that both $q(t)$ and $U(t)$ depend only on $\rho$ and the value of the random variable $X_{t}$. This implies that regardless of the state of the system in round $t-1$, by setting relative link load $\rho$ to the same value, the sender can achieve the same profile (or probability distribution) for $q(t)$ and $U(t)$. \ma{Confusing because $\rho$ obviously depends on the state in the previous round as well.} We will leverage this fact throughput our analysis.

\begin{lemma}
The function $g^f(\cdot)$ and the set $\mathbb{C}^f$ are convex for any positive PDF function $f$, where $f(x)=0$ for all $x \leq 0$.
\label{lemma:model1:convexity_of_bound}
\end{lemma}
\begin{proof}
See Appendix~\ref{app:model1:perfbound}.
\end{proof}


%\begin{lemma}
%In the model \S\ref{ss:model1:model}, for any causal congestion %control protocol, for any $t \in \mathbb{N}$, the point \{$E[q(t)]$, %$E[U(t)]$\} always lies in the convex set $\mathbb{C}^f$.
%\end{lemma}


\if 0
\begin{align}
        q(t) &= \frac{(Q(t-1) + s(t) \cdot T - \mu(t) \cdot T)^+}{\mu(t)}= T \cdot \left(\frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1) \cdot X_t} - 1 \right)^+\nonumber\\
        U(t) &= \frac{(\mu(t) \cdot T - s(t) \cdot T - Q(t - 1))^+}{\mu(t) \cdot T} = \left( 1 - \frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1) \cdot X_t}\right)^+
    \label{eq:model1:proof_perfbound:system}
\end{align}
Let's define a new variable $\rho(t)$ in terms of $Q(t-1)$, $s(t)$ and $\mu(t-1)$,
\begin{align}
  \rho =  \frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1)}  
\label{eq:model1:proof_perfbound:rt}
\end{align}

Intuitively, $\rho(t)$ can be thought of as the load on the link in time step $t$ relative to the link capacity in previous time step $\mu(t-1)$. Rewriting Eq. ~\eqref{eq:model1:proof_perfbound:system},
\begin{align}
    q(t) &= T \cdot \left(\frac{\rho}{X_t} - 1 \right)^+ &U(t) = \left(1 - \frac{\rho}{X_t}\right)^+
    \label{eq:model1:proof_perfbound:qU_rt}
\end{align}
\fi

To compute $E[q(t)]$ and $E[U(t)]$, we will first condition on the value of $\rho(t)$: 
\begin{align}
    E[q(t)|\rho(t)=b] &= E[T \cdot \left(\frac{b}{X_t} - 1 \right)^+] = T \cdot \int_{0}^{b}\left(\frac{b}{a} - 1 \right) \cdot f(a) \cdot da,\nonumber\\
                        %&= T \cdot \int_{0}^{z}\left(\frac{z}{x} - 1 \right) \cdot f(x) \cdot dx & \text{where } z=\rho\nonumber\\
    E[U(t)|\rho(t)=b] &= E[\left( 1 - \frac{b}{X_t}\right)^+] = \int_{b}^{\infty}\left( 1 - \frac{b}{a}\right) \cdot f(a) \cdot da.
\label{eq:model1:proof_perfbound:single_round_givenrt}
\end{align} 
Notice that Eq.~\eqref{eq:model1:proof_perfbound:single_round_givenrt} is identical to the curve $g^f$ from Eq.~\eqref{eq:model1:thm:perfbound}, i.e., the point $(E[q(t)|\rho(t)=b], E[U(t)|\rho(t)=b])$ lies on the curve $g^f$. Indeed, as we vary $b \in \mathbb{R}^+$, this point traces the entirety of $g^f$.

\if 0
%As we would expect, increasing the rate we send, in an uncertain environment, poses a direct trade-off between underutilization and queuing delay. 
%Increasing $\rho$ increases the conditional expected value of $q(t)$ and reduces the expected value of $U(t)$ . Varying $\rho$ in the above Eq. gives us the performance bound for round $t$.%curve between the two values. 

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/roundt_uniform.pdf}
    \vspace{-4mm}
    \caption{\small Trade-off between conditional expectation in a given time step t. $X \sim \textit{U}(0.27, 2) $, $T = 0.1$s. The color of the line corresponds to different values of $\rho=y$.}
    \label{fig:roundt_uniform}
    \vspace{-4.5mm}
 \end{figure}
\Fig{roundt_uniform} shows this trade-off curve for same distribution as \Fig{feasible_uniform}. 
\fi

%Since $\rho$ is a random variable it has a distribution dependent on the congestion strategy. 
Let the PDF of $\rho$ be $f_{r_t}$ in time step $t$. This distribution depends on the congestion control strategy and can be different for different time steps.  We have:
\begin{align}
    E[q(t)] &= E_{\rho(t)}[E[q(t)|\rho(t)]] = \int_{b=0}^{\infty}E[q(t)|\rho(t)=b]\cdot f_{r_t}(b) \cdot db,\nonumber\\
    E[U(t)] &= E_{\rho(t)}[E[U(t)|\rho(t)]] = \int_{b=0}^{\infty}E[U(t)|\rho=b] \cdot f_{r_t}(b) \cdot db.
\label{eq:model1:single_round}
\end{align}

Eq.~\eqref{eq:model1:single_round} shows that the point $(E[q(t)], E[U(t)])$ is a weighted average of the points $(E[q(t)|\rho(t)=b], E[U(t)|\rho(t)=b])$ for different values of $b$, all of which lie on the curve $g^f$. The actual value of $(E[q(t)], E[U(t)])$ depends on the distribution $f_{r_t}$, which determines the weight given to each point on $g^f$. But regardless of $f_{r_t}$, the point $(E[q(t)], E[U(t)])$ will lie in the set $\mathbb{C}^f$ since $g^f$ is convex.

%The actual value of the point $\{E[q(t)], E[U(t)]\}$ will depend on the distribution $fr^t$. Regardless of $fr^t$, the point $\{E[q(t)], E[U(t)]\}$ is a weighted average (with $fr^t(b)$ as weights) of points $\{E[q(t)|\rho=b], E[U(t)|\rho=b]\}$ with different values of $b$, all of which lie on the curve $g^f$. Since $g^f$ is convex with increasing slope, for any $fr^t \in \mathbb{R}^+ \to \mathbb{R}^+ $ (i.e., for any causal congestion control strategy), the point $\{E[q(t), E[U(t)\}$  will lie in the set $\mathbb{C}^f$. Lemma proved.

Finally, let us consider the expected queuing delay and underutilization over multiple time steps: 
\begin{align}
    E[\bar{q}(t)] &= E\left[\frac{\sum_{i=1}^{t}q(i)}{t}\right] = \frac{\sum_{i=1}^{t}E[q(i)]}{t}, & E[\bar{U}(t)] &= E\left[\frac{\sum_{i=1}^{t}U(i)}{t}\right] = \frac{\sum_{i=1}^{t}E[U(i)]}{t}.
\end{align}
The point $(E[\bar{q}(t)], E[\bar{U}(t)])$ is the average of the points $(E[q(i)], E[U(i)])$ for $1 \leq i \leq t$. Since all these points belong to the convex set $\mathbb{C}^f$, their average must also lie in the set $\mathbb{C}^f$. This completes the proof. \qed

 \subsection{Is the Performance Bound Achievable?}
 \label{ss:model1:achievable_bound}
The analysis in the previous section provides insight into how to achieve a particular point on performance bound. The key observation is that we need to maintain the same ``load'' $\rho(t)$ in every time step. Recall that $\rho(t)$ determines the operating point $(E[q(t)], E[U(t)])$ achieved on the curve $g^f$ in each time step. If $\rho(t)$ changes from round to round, then over multiple time steps we will end up at a sub-optimal point in the interior of $\mathbb{C}^f$. However, if the congestion control algorithm can keep $\rho(t)$ constant over time, it can achieve an optimal tradeoff between underutilization and queuing delay.

Setting $\rho(t) = C$ (for some constant $C$) in Eq.~\eqref{eq:model1:proof_perfbound:rt} suggests the following control law: 
\begin{align}
    s(t) &= C \cdot \mu(t-1) - \frac{Q(t-1)}{T}, \quad \forall t \in \mathbb{N}.
    \label{eq:simple-rule}
\end{align}
%where $E[q(t)|\rho(t)=C]=x$.%$C \in R+$. 
The first term selects a sending rate proportional to the current link capacity $\mu(t-1)$. This is an intuitive choice since the next capacity $\mu(t)$ is also proportional to $\mu(t-1)$ (albeit with an unknown multiplicative factor). The second term deducts a rate based on the current queue backlog from the sending rate. This deduction corresponds to the rate necessary to drain the current queue backlog within one time step. The parameter $C$ controls the tradeoff between underutilization and queuing delay. As $C$ increases, the congestion control sends more aggressively, favoring high utilization at the expense of queuing delay. This corresponds to moving to the right on the curve $g^f$ (see Fig.~\ref{fig:model1:feasible_uniform}).

However, it may not always be possible to strictly follow the above rule. In Eq.~\eqref{eq:simple-rule}, $s(t)$ can become negative, but of course the sending rate must be non-negative. For example, it might so happen by chance that the link capacity drops rapidly over a number of consecutive time steps, leading to a large queue build up. If in any time step $t$, $Q(t-1)$ exceeds $T \cdot C \cdot \mu(t-1)$, then the sender will have to pick a negative sending rate to follow $\rho(t) = C$, which is not possible. 

This argument shows that depending on the distribution $f$ of the link variation and the value $C$, it may not be possible to achieve some  points on the curve $g^f$. This is more likely for high values of $C$, which makes the controller more aggressive, and for distributions $f$ where the link capacity can drop significantly each time step. The following proposition gives sufficient necessary conditions on $C$ such that the sender can always follow the rule in Eq.~\eqref{eq:simple-rule} and enforce $\rho(t)=C$. 

%In particular, if $Q(t-1) > T \cdot C \cdot \mu(t-1)$, then under this strategy $s(t) < 0$ (not possible).

%In such a scenario, the point $\{E[\bar{q}(t]$, $E[\bar{U}(t)]\}$) might not be on the boundary of set $\mathbb{C}^f$. 

%The points on the trade-off boundary correspond to $\rho = C_r, \forall t \in t_{range}$. From Eq.. ~\ref{eq:model1:proof_perfbound:rt}, it implies that the sending rate $s(t)$ must be equal to $C_r \cdot \mu(t-1) - \frac{Q(t-1)}{T}, \forall t \in t_{range}$ for us to be on the boundary. If the $Q(t-1)$ become high ($> T \cdot C_r \cdot \mu(t-1)$, because of say variations in the link capacity), then $s(t)$ will have to be negative, which is not possible. %\tom{not obvious that this follows! You derived that Cr is constant under an assumption that s(t) could be negative.  So its not clear that there is still a Cr if s(t) cannot be negative.  If we constrain s(t) to non-negative values, leaving Cr constant, then in any round, \rho > Cr.}\pg{I have not assumed anything. I am simply saying the point on the trade-off boundary corresponds to $\rho = C_r$ in every round. Then the question I am asking is a sending rate policy that gives you $\rho =C_r$ possible? The answer depends on the $C_r$ you are choosing and the bounds on variation in the link model itself.} 
%As a result, $\rho > C_r$, and the trade-off point will be inside the boundaries.
 
%\tom{more explanation needed here too.  You are deriving constraints on the PDF f, such that the above solution holds (i think). You need to say that.  And I'm not sure, retrospectively, if it wouldn't be better for you to simply say, early on, that we constrain f in such as a way as the solution is feasible.  The form of that constraint is derived here.  But doesn't the constraint on f depend in a very direct way on our choice of Cr?  And so Cr isn't really a constant?  That is, if we find ourselves falling behind, might we decide to change Cr before we become unfeasible?} 

%We will now establish the conditions on $C$ under which the sender can follow $\rho(t) = C$. In particular, we will show that as long as $C$ is smaller than a threshold, the sender can follow the control law exactly.


\begin{proposition}
In the MIF model, it is possible to follow the strategy $\rho(t) = C$,  $\forall t \in \mathbb{N}$ iff
\begin{align}
    C &\leq \frac{X_{min}}{1 - X_{min}},
    \label{eq:prop:model1:achievable_bound}
\end{align}
where $X_{min}$ is the minimum value of the random variable $X$ ($P(X<X_{min}) = 0$). 
\label{prop:model1:achievable_bound}
\end{proposition} 
\begin{proof}
Please see Appendix~\ref{app:model1:prop}
\end{proof}

\if 0
\begin{proof}

\ma{I think this proof could go into the appendix. This proposition isn't central to the story.} \pg{Will move.}

We will prove this by induction. We will show that if the above condition holds then with the policy $\rho(t) = C$, $Q(t)  \leq T \cdot C \cdot \mu(t)$ $\forall t \in \mathbb{N}$.  

The base case holds because $Q(0) = 0$. Lets assume that $Q(t - 1) 
 \leq T \cdot C \cdot \mu(t-1)$, then we can pick a non negative $s(t)$, such that $\rho(t) = C$. Then in the next round $t$,
 \begin{align}
     Q(t) &= (Q(t-1) + s(t) \cdot T- \mu(t) \cdot T)^+,\nonumber\\
          &= (T \cdot C \cdot \mu(t - 1) - T \cdot \mu(t))^+,\nonumber\\
          &=  T \cdot C \cdot \mu(t) \cdot (\frac{1}{X_t} - \frac{1}{C})^+, \nonumber\\
          &\leq T \cdot C \cdot \mu(t) \cdot (\frac{1}{X_{min}} - \frac{1}{C})^+,\nonumber\\
          &\leq T \cdot \mu(t) \cdot C,
 \end{align}
 where in the last step we used Eq.~\eqref{eq:prop:model1:achievable_bound}.
\end{proof}
\fi
%Notice that this condition is dependent on the value of $X_{min}$. Lower $X_{min}$ implies that the link capacity can reduce by a higher amount and it is more likely for the sender to build an excessive queue.

This analysis shows us that the performance bound need not be tight. For any $f(\cdot)$, the points $(x, g^f(x))$ where $E[q(t)|\rho(t)=C] = x$ but $C$ does not meet the condition above might not be achievable. %\ma{This implies that the condition in Prop. 1 is actually an ``if only if'' condition. But we didn't show that right? Leaving this here until we resolve this comment. } \pg {I think if the above condition is violated with some probability the sender \emph{will} have to pick a higher $r(t) = C_1$ > $C$ some time. But if a portion of curve $g^f$ is a straight line then it might still be possible to achieve the desired trade-off exactly.}

\subsection{Optimal Control Law}
\label{ss:model1:mdp}

What happens when the above condition is not met and $Q(t-1)$ can exceed $T \cdot C \cdot \mu(t-1)$? A natural question to ask is: in the event of excessive queuing, should the sender just pick the minimum value for $\rho(t)$ such that $s(t)$ is non-negative? This corresponds to $\rho(t) = \max(C, \frac{q(t-1)}{T})$, which implies a control law of the following form:
\begin{align}
    s(t) &= (C \cdot \mu(t-1) - \frac{Q(t-1)}{T})^+, \quad \forall t \in \mathbb{N}.
\end{align}

We now show that the above rule can indeed achieve an optimal tradeoff between underutilization and queuing delay. To this end, we formulate the congestion control task as a Markov Decision Process~\cite{sutton2018reinforcement} (MDP) and show that the above rule is an optimal policy for this MDP. 

The MDP is defined as follows. The {\em state} at time step $t$ is given by $(q(t-1), \mu(t-1))$. The congestion control ``agent'' observes this state and selects an {\em action}\,---\,the sending rate $s_t \geq 0$. The state then transitions to the next state $(q(t), \mu(t))$, and the agent incurs a weighted {\em cost} $(w\cdot q(t) + U(t))$ for this time step, depending on the relative importance of low queuing delay versus low underutilization. To see that this is an MDP, recall that the transitions occur according to:
\begin{align}
    \mu(t)&=\mu(t-1)\cdot X_t \quad \text{(per the MIF model)}, \nonumber\\
    q(t)&=T\cdot(\rho(t)/X_t-1)^+ \quad \text{(per Eq.~\eqref{eq:model1:proof_perfbound:qU_rt})}, \nonumber
\end{align} 
Therefore the next state is determined by the current state and the congestion control action, since $\rho(t) =  \frac{q(t-1)\mu(t-1)+T\cdot s(t)}{T\cdot \mu(t-1)}$  (Eq.~\eqref{eq:model1:proof_perfbound:rt}).

The agent uses a control policy $\pi$ mapping the current state to a probability distribution over possible actions (i.e., sending rates $s(t)\geq 0$). The policy can be deterministic or stochastic. The goal of the agent is to minimize the following objective function over all policies:
\begin{align}
     J(\pi) = E\left[\sum_{t=1}^{\infty}\gamma^{t-1} \Big( w \cdot q(t) + U(t)] \Big)\right].
\label{eq:model1:mdp:objective}
\end{align}
Here we use a standard discounted cost formulation, with discount factor $\gamma \in (0,1)$.

\begin{theorem}
    In the MDP defined above, the optimal control policy that minimizes $J(\pi)$ takes the form:  
    \begin{align}
        s(t) = \left( C(w, \gamma) \cdot \mu(t-1) - \frac{Q(t-1)}{T} \right)^+,  
        \label{eq:thm:model1:mdp}
    \end{align}
where $C(w,\gamma)$ is a constant. 
    \label{thm:model1:mdp}
\end{theorem}
\begin{proof}
Define the optimal value function~\cite{sutton2018reinforcement} for our MDP as:
\begin{align}
    V(q,\mu) = \min_\pi E\left[\sum_{t=1}^{\infty}\gamma^{t-1} \Big( w \cdot q(t) + U(t)] \Big) \;\middle|\; q(0) = q, \mu(0) = \mu, s(t) \sim \pi(\cdot|q(t-1),\mu(t-1))\right]. 
\end{align}
This is the minimum possible discounted expected sum of costs, starting from initial state $(q,\mu)$ and following policy $\pi$, over all policies $\pi$.\footnote{We only consider $f(\cdot)$ for which $V(q,\mu)$ exists. Otherwise, if $V(q,\mu) \to \infty$, then for the state $(q, \mu)$, every control law has the same value function ($\infty$) and the optimal control law is not defined. \ma{As defined, we only talk about the optimal value function, which doesn't depend on a specific policy, so this could be confusing. Can we this say something like: if $V(q,\mu) = \infty$ for some states $(q, \mu)$, then it is easy to show that $V(q,\mu) = \infty$ for {\em every}) state $(q, \mu)$ with $q \neq 0$, and therefore the problem becomes meaningless.} \pg{I don't think this statement is true.} \ma{but i also don't see why $V(q,\mu)$ infinity for one state can imply anything about the optimal control law being undefined. hypothetically the optimal law would try to avoid that state!} \pg{I was wondering if we could formulate the objective function in itself as a function of the state of the system. then this goes away. If we do this we might have to get rid of the assumption Q(0) = 0.} \pg{alternatively we could get rid of the footnote altogether.}} %See discussion in Appendix~\ref{appxxx}. $\sum_{k\geq 1} \gamma^k E[(1/X)]^k  < $ => $\gamma E(1/X) < 1 $}

The optimal value function satisfies the following Bellman Equation:
\begin{align}
    V(q,\mu) = \min_{s(1) \geq 0} E \left[ w\cdot q(1) + U(1) + \gamma V(q(1), \mu(1)) \;\middle|\; q(0) = q, \mu(0) = \mu \right]. 
\end{align}
The condition $s(1) \geq 0$ is equivalent to $\rho(1) \geq q/T$. Rewriting,  
\begin{align}
    V(q,\mu) = \min_{\rho(1) \geq \frac{q}{T}} E \left[ w\cdot q(1) + U(1) + \gamma V(q(1), \mu(1)) \;\middle|\; q(0) = q, \mu(0) = \mu \right]. 
\end{align}

\begin{lemma}
$V(q,\mu)$ is a convex function of $q$ and does not depend on $\mu$. 
\label{lemma:model1:combined_mdp_lemma}
\end{lemma}
\begin{proof}
See Appendix~\ref{app:model1:combined_mdp_lemma}.
\end{proof}
Since $V$ does not depend on $\mu$, henceforth we will write the optimal value function as $V(q)$. To complete the proof, we exploit the fact that $q(t)$ and $U(t)$ only depend on the value of $\rho(t)$ and define a helper function $W(\cdot)$ as follows,
\begin{align}
    W(\rho) &= E\left[ w \cdot q(1) + U(1) + \gamma \cdot V(q(1)) \;\middle|\; \rho(1) = \rho\right], & V(q) &= \min_{\rho \geq \frac{q}{T}} (W(\rho)).
    %W_{t}(\rho(t))  &= \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t+1}(T \cdot (\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg), & \forall t \leq n, \nonumber\\
    %V_{t}^2(\rho(t)) &= \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    %&+ \int_{0}^{\infty}f(a) \cdot V_{t-1}^1((\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg)\nonumber &, \forall t<n\nonumber\\
    \label{eq:model1:mdp_helper_def}
\end{align}
$W(\rho)$ is the minimum expected cost when we restrict the first action to $\rho(1) = \rho$ and then act optimally from that step onward.  

\begin{lemma}
    $W(\rho)$ is a convex function in $\rho$.
\end{lemma}
\begin{proof}
The proof directly follows from proof of Sub lemma~\ref{sublemma:model1_helper} in Appendix~\ref{app:model1:combined_mdp_lemma}.
\end{proof}

Let the minimum value of $W(\cdot)$ occur at $\rho^*$. Then, the convexity of $W(\cdot)$ combined with Eq.~\eqref{eq:model1:mdp_helper_def} establishes that the optimal control law is of the form $\rho(t) = \max(\rho^*, q(t-1)/T)$. To see this, note that the minimizer of $W(\rho)$ in Eq.~\eqref{eq:model1:mdp_helper_def} is $\rho = q/T$ if $\rho^* < q/T$, and $\rho = \rho^*$ otherwise. Furthermore, note that $\rho^*$ depends on $\gamma$ and $w$. Defining $C(w, \gamma) = \rho^*$ and using Eq.~\eqref{eq:model1:proof_perfbound:rt} we get the optimal control law from the Theorem. 

\end{proof}



%To answer this question, we formulate the problem as markov decision process (MDP) over a finite number of rounds $n$. In particular our goal is to find a causal congestion control strategy which minimizes the value of the following objective function in each round,
%\begin{align}
% \sum_{i=t}^{n}\gamma^{i-t} \Big( w \cdot E[q(i)] + E[U(i)] \Big), && \forall t \leq n,
%\end{align}
%where $\gamma$ is the standard discount factor and $\gamma \in (0,1)$. Here, we introduce the discount factor so that we can later extend our analysis to infinite horizon ($n \to \infty$).
%\pg{Technically our proof holds for any objective convex function in terms of E[q(i)] and E[U(i)]. Include this statement?}



% $C$ for which the above condition is not met, we conjecture the following strategy, $\rho(t) = max(C_r, \frac{Q(t-1)}{T \cdot \mu(t-1)})$ or $s(t) = (\mu(t-1) \cdot C_r - \frac{Q(t-1)}{T})^+$ will be optimal.

%We will now prove the above conjecture by modelling the system as a Markov Decision Process (MDP), where the goal is to pick a sending rate strategy to minimize $w \cdot E[\frac{\bar{q}(t)}{T}] + E[\bar{U}(t)]$. %\ma{Start by defining the MDP, and I think it would be better to drop the $1/T$ in the definition of the objective and value functions}  

\if 0

We will now write the Bellman Equation governing this optimization problem. Where $V_{t-1}(\cdot)$\cut{$q(t-1),\mu(t-1))$} is the value function at time step $t-1$.
\begin{align}
    V_{t-1}(q(t-1),\mu(t-1)) &= \min_{s(t) \geq 0} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot E[V_{t}(q(t),\mu(t))]\Bigg) \nonumber, & \forall t \leq n,\\
    V_{t-1}(q(t-1),\mu(t-1)) &= \min_{s(t) \geq 0} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(q(t),\mu(t)) \cdot da\Bigg), \nonumber & \forall t \leq n,\\
   V_{t}(q(t),\mu(t)) &= 0, & t=n.
\end{align}

The condition $s(t)\geq 0$ is equivalent to $\rho(t)\geq\frac{q(t-1)}{T}$. Rewriting,
\begin{align}
    V_{t-1}(q(t-1),\mu(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(q(t), \mu(t)) \cdot da\Bigg), & \forall t \leq n.\nonumber\\
     %V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
     \label{eq:model1:conjecture}
\end{align}

In the equation above, the first two terms on the right hand side ($w \cdot E[q(t)] and E[U(t)]$) depend only on the value of $\rho(t)$. Since $q(t)$ only depends on $\rho(t)$, this implies that if $V_{t}(\cdot)$ is only a function of $q(t)$ and independent of $\mu(t)$, then $V_{t-1}(\cdot)$ is also only a function of $q(t-1)$. Since $V_{n}(\cdot)$ is independent of $\mu(n)$, $\forall t < n$ we can describe the function $V_{t-1}(\cdot)$ using only $q(t-1)$. Rewriting equations,  

\begin{align}
    V_{t-1}(q(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(T \cdot (\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg), & \forall t \leq n.\nonumber\\
    % V_{t-1}^1(\frac{q(t-1)}{T}) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
    \label{eq:model1:v_def}
\end{align}

%Since the quantity over which we are taking the minima only depends on $\rho(t)$, $V_t$ is non-decreasing. 
To help our analysis, we define a new helper function  $V_{t}^2(
\cdot)$ as follows,
\begin{align}
    V_{t}^2(\rho(t))  &= \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(T \cdot (\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg), & \forall t \leq n, \nonumber\\
    V_{t-1}(q(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} (V_{t}^2(\rho(t))), & \forall t \leq n. \nonumber\\
    %V_{t}^2(\rho(t)) &= \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    %&+ \int_{0}^{\infty}f(a) \cdot V_{t-1}^1((\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg)\nonumber &, \forall t<n\nonumber\\
\end{align}

%Consequently, the best strategy in a given round $t$ is of the form $\rho(t) = C(t)$ or $s(t) = max\left(0, C(t) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)$. 

%\todo{To show that the best strategy in every round is the same we need to show that the value function in every round is the same.} \pg{Not sure if the math in comments below to prove For all t, $V_{t-1}$ is convex is required at all?}

We will now show that both $V_{t-1}(\cdot)$ and $V_{t}^2(\cdot)$ are convex.
\begin{lemma}
$\forall t \leq n$, both $V_{t-1}(\cdot)$ and $V_{t}^2(\cdot)$ are convex.
\label{lemma:model1:mdp_convex}
\end{lemma}
We give an induction based proof for the Lemma (see Appendix ~\ref{app:model1:mdp_convex_lemma}). Our proof exploits the fact that both $E[q(t)|\rho(t)]$ and $E[U(t)|\rho(t)]$ are both convex in $\rho(t)$.

The convexity property establishes that best strategy in any given time step $t$ is of the following form,
\begin{align}
\rho(t) &= max(C(w,t), \frac{q(t-1)}{T}), & s(t) = \left(C(w, t) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)^+, 
\end{align}
where the minimum value of $V^2_{t}(\cdot)$ occurs at $\rho(t) = C(w, t)$ or $V_{t-1}(0) = V^2_{t}(C(w, t))$. 
We can calculate the exact value of $C(w, t)$ by solving the Bellman equation to calculate the functions $V_{t-1}(\cdot), V^2_t(\cdot)$ starting from round $n$ and working backwards.

%\pg{intuition why is it convex and why is it useful.}

\todo{Feedback NEEDED. To show that the best strategy in every round is the same we need to show that the value function in every round is the same.} %With the conjecture strategy we get a convex feasible set.}

Next, we consider this MDP over infinite horizon.

\begin{conjecture}
    As $n \to \infty$, $V_{t_1-1}(x) \to V_{0}(x)$ and $V_{t_1}^2(x) \to V_{1}^2(x), \forall t_1 << n$ and $x \in \mathbb{R}^+$.
    \label{conj:model1:value_function}
\end{conjecture}


\pg{How to prove this conjecture? Do we need to? Is giving an intuition like the following enough?} 

Informally, the conjecture if arguing that the value functions converge as $n \to \infty$. The intuition for this conjecture is as follows.  Consider the strategy ($CS$), where 
\begin{align}
    \rho(t) &= max(C(w,t + (t_1-1)),\frac{q(t-1)}{T}), & \forall t \in [1, n-(t_1-1)], \nonumber\\
    \rho(t) &= max(C(w,t), \frac{q(t-1)}{T}), &\forall t \in (n-(t_1-1), n].
\end{align}
. 

If the sender follows this strategy instead of the optimal, then we get,
\begin{align}
    V_{0}(x) \leq V_{t_1-1}(x) + \gamma^{n-t_1+1} E_{CS, x}[V_{n-(t_1-1)}(q(n-(t_1-1)))].
\end{align}

Similarly consider the following strategy,
\begin{align}
    %\rho(t) &= max(C(w,t),\frac{q(t-1)}{T}) &, \forall t \in [1, t_1)
    \rho(t) &= max(C(w,t + (1-t_1)),\frac{q(t-1)}{T}), & \forall t \in [t_1, n].
\end{align}
If the sender follows this strategy instead of the optimal, then we get,
\begin{align}
    V_{t_1-1}(x) \leq V_{0}(x).
\end{align}

As $n \to \infty$, $\gamma^{n-t_1+1} \to 0$. If $E_{CS, x}[V_{n-(t_1-1)}(q(n-(t_1-1)))]$ is finite then we get,  $V_{t_1-1}(x) \to V_{0}(x)$.

\begin{theorem}
    In the model~\S\ref{ss:model1:model}, for the MDP~\S\ref{ss:model1:mdp}, if Conjecture~\ref{conj:model1:value_function} holds, then as $n \to \infty \forall t << n$, the following causal congestion control protocol is optimal. 
    \begin{align}
        s(t) = \left( C(w) \cdot \mu(t-1) - \frac{Q(t-1)}{T} \right)^+,  
        \label{eq:thm:model1:mdp}
    \end{align}
    \label{thm:model1:mdp}
\end{theorem}
where $V_{0}(0) = V^2_{1}(C(w))$.

Proof: Directly follows from Conjecture~\ref{conj:model1:value_function}.

This theorem establishes that for all rounds, the sender should try to keep the relative link load constant ($\rho(t) = C(w)$). In the event of excessive queuing ($q(t-1) > T \cdot C(w))$), the sender should pick the minimum possible value for relative link load ($\rho(t) = \frac{q(t-1)}{T}$ or $s(t) = 0$).

\fi
%\pg{Give mathematical intuition and implication everywhere.}



\if 0
\subsection{Optimal Control Law}
\label{ss:model1:mdp}

What happens when the above condition is not met and $Q(t-1)$ can exceed $T \cdot C \cdot \mu(t-1)$? A natural question to ask is: in the event of excessive queuing, should the sender just pick the minimum value for $\rho(t)$ such that $s(t)$ is non-negative? This corresponds to $\rho(t) = max(C, \frac{q(t-1)}{T})$, which implies a control law of the following form:
\begin{align}
    s(t) &= (C \cdot \mu(t-1) - \frac{Q(t-1)}{T})^+, \quad \forall t \in \mathbb{N}.
\end{align}

To answer this question, we formulate the problem as markov decision process (MDP) over a finite number of rounds $n$. In particular our goal is to find a causal congestion control strategy which minimizes the value of the following objective function in each round,
\begin{align}
 \sum_{i=t}^{n}\gamma^{i-t} \Big( w \cdot E[q(i)] + E[U(i)] \Big), && \forall t \leq n,
\end{align}
where $\gamma$ is the standard discount factor and $\gamma \in (0,1)$. Here, we introduce the discount factor so that we can later extend our analysis to infinite horizon ($n \to \infty$).
\pg{Technically our proof holds for any objective convex function in terms of E[q(i)] and E[U(i)]. Include this statement?}



% $C$ for which the above condition is not met, we conjecture the following strategy, $\rho(t) = max(C_r, \frac{Q(t-1)}{T \cdot \mu(t-1)})$ or $s(t) = (\mu(t-1) \cdot C_r - \frac{Q(t-1)}{T})^+$ will be optimal.

%We will now prove the above conjecture by modelling the system as a Markov Decision Process (MDP), where the goal is to pick a sending rate strategy to minimize $w \cdot E[\frac{\bar{q}(t)}{T}] + E[\bar{U}(t)]$. %\ma{Start by defining the MDP, and I think it would be better to drop the $1/T$ in the definition of the objective and value functions}  

We will now write the Bellman Equation governing this optimization problem. Where $V_{t-1}(\cdot)$\cut{$q(t-1),\mu(t-1))$} is the value function at time step $t-1$.
\begin{align}
    V_{t-1}(q(t-1),\mu(t-1)) &= \min_{s(t) \geq 0} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot E[V_{t}(q(t),\mu(t))]\Bigg) \nonumber, & \forall t \leq n,\\
    V_{t-1}(q(t-1),\mu(t-1)) &= \min_{s(t) \geq 0} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(q(t),\mu(t)) \cdot da\Bigg), \nonumber & \forall t \leq n,\\
   V_{t}(q(t),\mu(t)) &= 0, & t=n.
\end{align}

The condition $s(t)\geq 0$ is equivalent to $\rho(t)\geq\frac{q(t-1)}{T}$. Rewriting,
\begin{align}
    V_{t-1}(q(t-1),\mu(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(q(t), \mu(t)) \cdot da\Bigg), & \forall t \leq n.\nonumber\\
     %V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
     \label{eq:model1:conjecture}
\end{align}

In the equation above, the first two terms on the right hand side ($w \cdot E[q(t)] and E[U(t)]$) depend only on the value of $\rho(t)$. Since $q(t)$ only depends on $\rho(t)$, this implies that if $V_{t}(\cdot)$ is only a function of $q(t)$ and independent of $\mu(t)$, then $V_{t-1}(\cdot)$ is also only a function of $q(t-1)$. Since $V_{n}(\cdot)$ is independent of $\mu(n)$, $\forall t < n$ we can describe the function $V_{t-1}(\cdot)$ using only $q(t-1)$. Rewriting equations,  

\begin{align}
    V_{t-1}(q(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(T \cdot (\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg), & \forall t \leq n.\nonumber\\
    % V_{t-1}^1(\frac{q(t-1)}{T}) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
    \label{eq:model1:v_def}
\end{align}

%Since the quantity over which we are taking the minima only depends on $\rho(t)$, $V_t$ is non-decreasing. 
To help our analysis, we define a new helper function  $V_{t}^2(
\cdot)$ as follows,
\begin{align}
    V_{t}^2(\rho(t))  &= \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f(a) \cdot V_{t}(T \cdot (\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg), & \forall t \leq n, \nonumber\\
    V_{t-1}(q(t-1)) &= \min_{\rho(t) \geq \frac{q(t-1)}{T}} (V_{t}^2(\rho(t))), & \forall t \leq n. \nonumber\\
    %V_{t}^2(\rho(t)) &= \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    %&+ \int_{0}^{\infty}f(a) \cdot V_{t-1}^1((\frac{\rho(t)}{a} - 1)^+) \cdot da\Bigg)\nonumber &, \forall t<n\nonumber\\
\end{align}

%Consequently, the best strategy in a given round $t$ is of the form $\rho(t) = C(t)$ or $s(t) = max\left(0, C(t) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)$. 

%\todo{To show that the best strategy in every round is the same we need to show that the value function in every round is the same.} \pg{Not sure if the math in comments below to prove For all t, $V_{t-1}$ is convex is required at all?}

We will now show that both $V_{t-1}(\cdot)$ and $V_{t}^2(\cdot)$ are convex.
\begin{lemma}
$\forall t \leq n$, both $V_{t-1}(\cdot)$ and $V_{t}^2(\cdot)$ are convex.
\label{lemma:model1:mdp_convex}
\end{lemma}
We give an induction based proof for the Lemma (see Appendix ~\ref{app:model1:mdp_convex_lemma}). Our proof exploits the fact that both $E[q(t)|\rho(t)]$ and $E[U(t)|\rho(t)]$ are both convex in $\rho(t)$.

The convexity property establishes that best strategy in any given round $t$ is of the following form,
\begin{align}
\rho(t) &= max(C(w,t), \frac{q(t-1)}{T}), & s(t) = \left(C(w, t) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)^+, 
\end{align}
where the minimum value of $V^2_{t}(\cdot)$ occurs at $\rho(t) = C(w, t)$ or $V_{t-1}(0) = V^2_{t}(C(w, t))$. 
We can calculate the exact value of $C(w, t)$ by solving the Bellman equation to calculate the functions $V_{t-1}(\cdot), V^2_t(\cdot)$ starting from round $n$ and working backwards.

%\pg{intuition why is it convex and why is it useful.}

\todo{Feedback NEEDED. To show that the best strategy in every round is the same we need to show that the value function in every round is the same.} %With the conjecture strategy we get a convex feasible set.}

Next, we consider this MDP over infinite horizon.

\begin{conjecture}
    As $n \to \infty$, $V_{t_1-1}(x) \to V_{0}(x)$ and $V_{t_1}^2(x) \to V_{1}^2(x), \forall t_1 << n$ and $x \in \mathbb{R}^+$.
    \label{conj:model1:value_function}
\end{conjecture}


\pg{How to prove this conjecture? Do we need to? Is giving an intuition like the following enough?} 

Informally, the conjecture if arguing that the value functions converge as $n \to \infty$. The intuition for this conjecture is as follows.  Consider the strategy ($CS$), where 
\begin{align}
    \rho(t) &= max(C(w,t + (t_1-1)),\frac{q(t-1)}{T}), & \forall t \in [1, n-(t_1-1)], \nonumber\\
    \rho(t) &= max(C(w,t), \frac{q(t-1)}{T}), &\forall t \in (n-(t_1-1), n].
\end{align}
. 

If the sender follows this strategy instead of the optimal, then we get,
\begin{align}
    V_{0}(x) \leq V_{t_1-1}(x) + \gamma^{n-t_1+1} E_{CS, x}[V_{n-(t_1-1)}(q(n-(t_1-1)))].
\end{align}

Similarly consider the following strategy,
\begin{align}
    %\rho(t) &= max(C(w,t),\frac{q(t-1)}{T}) &, \forall t \in [1, t_1)
    \rho(t) &= max(C(w,t + (1-t_1)),\frac{q(t-1)}{T}), & \forall t \in [t_1, n].
\end{align}
If the sender follows this strategy instead of the optimal, then we get,
\begin{align}
    V_{t_1-1}(x) \leq V_{0}(x).
\end{align}

As $n \to \infty$, $\gamma^{n-t_1+1} \to 0$. If $E_{CS, x}[V_{n-(t_1-1)}(q(n-(t_1-1)))]$ is finite then we get,  $V_{t_1-1}(x) \to V_{0}(x)$.

\begin{theorem}
    In the model~\S\ref{ss:model1:model}, for the MDP~\S\ref{ss:model1:mdp}, if Conjecture~\ref{conj:model1:value_function} holds, then as $n \to \infty \forall t << n$, the following causal congestion control protocol is optimal. 
    \begin{align}
        s(t) = \left( C(w) \cdot \mu(t-1) - \frac{Q(t-1)}{T} \right)^+,  
        \label{eq:thm:model1:mdp}
    \end{align}
    \label{thm:model1:mdp}
\end{theorem}
where $V_{0}(0) = V^2_{1}(C(w))$.

Proof: Directly follows from Conjecture~\ref{conj:model1:value_function}.

This theorem establishes that for all rounds, the sender should try to keep the relative link load constant ($\rho(t) = C(w)$). In the event of excessive queuing ($q(t-1) > T \cdot C(w))$), the sender should pick the minimum possible value for relative link load ($\rho(t) = \frac{q(t-1)}{T}$ or $s(t) = 0$).


%\pg{Give mathematical intuition and implication everywhere.}

\fi 

\section{Implications and Validation of the MIF model}
\label{ss:model1:implications}
%\pg{Regenerate graphs. Feedback on the legend name appreciated.}
In this section, we discuss some of the implications of the formal analysis given above. First, we validate our model against real cellular traces (Verizon LTE Uplink and Downlink) taken from earlier work~\cite{mahimahi}. Recall that the cellular traces need not follow our model. We also generate a synthetic trace based on the MIF model with $X \sim e^{\textit{U(-1, 1})}$ \ma{confusing organization of sentences. i can't tell if we mean the next two sentences are only for the synthetic traces and then the stuff that comes after that is for only the cellular traces or what.} 
\pg{For these traces, we plot the expected underutilization ($E[\bar{U}]$) versus the expected normalized queuing delay ($E(\bar{q})$). We compare the performance bound from Theorem~\ref{thm:model1:perfbound} and the optimal control law from Theorem~\ref{thm:model1:mdp}. 
We use the empirical distribution of values $\frac{\mu(t)}{\mu(t-1)}$ from the traces as our PDF $f$ to compute the performance bound and we simulate the optimal control law for different values of $C(w, \gamma)$. 
For the cellular traces, we also show the performance for various previously proposed congestion control algorithms.} 
We consider Cubic+Codel~\cite{cubic, CoDel}, XCP~\cite{xcp}, ABC~\cite{abc, goyal2017rethinking}, Sprout~\cite{sprout}, and Copa~\cite{copa} as representing the best performing alternatives. We emulate the traces using the Mahimahi network emulation tool~\cite{mahimahi}. For Copa and Sprout, we use the authors' UDP implementations.
For the Cubic endpoints, we use the Linux TCP implementation.
For Codel, XCP, and ABC, we use the implementation and configuration parameters from ~\cite{abc}. 
To make these systems comparable to the derived bounds, we compute the queuing delay once per baseline round trip.
\if 0
For these traces, we plot the expected underutilization ($E[\bar{U}]$) versus the expected normalized queuing delay ($E(\bar{q})$). We compare the performance bound from Theorem~\ref{thm:model1:perfbound}, the optimal control law from Theorem~\ref{thm:model1:mdp}, and various previously proposed congestion control algorithms. 
For the cellular traces, we use the empirical distribution of values $\frac{\mu(t)}{\mu(t-1)}$ from the traces as our PDF $f$ to compute the performance bound; we simulate the optimal control law for different values of $C(w, \gamma)$; and we consider Cubic+Codel~\cite{cubic, CoDel}, XCP~\cite{xcp}, ABC~\cite{abc, goyal2017rethinking}, Sprout~\cite{sprout}, and Copa~\cite{copa} as representing the best performing alternatives. We emulate the traces using the Mahimahi network emulation tool~\cite{mahimahi}. For Copa and Sprout, we use the authors' UDP implementations.
For the Cubic endpoints, we use the Linux TCP implementation.
For Codel, XCP, and ABC, we use the implementation and configuration parameters from ~\cite{abc}. 
To make these systems comparable to the derived bounds, we compute the queuing delay once per baseline round trip.
\fi
% \tom{are we including cubic? if not, presumably we aren't using the Linux TCP implementation?}\pg{We have cubic+Codel, end point is running cubic while the bottleleck router is using the codel scheme.}
% 

\Fig{model1:basic} shows our main result: it is possible to achieve a smooth tradeoff across a large range of
underutilization and queuing delay. There is a significant gap between the five 
existing congestion control algorithms and the performance of the optimal control law on the Verizon traces.
Note that the formatting differs from \Fig{intro_perf} in that the x-axis is linear rather than log scale. 
For the cellular
traces, there is only a small gap between the predicted performance bound and the optimal control law.  This difference
is larger in the case of the synthetic trace. To achieve very low levels of underutilization on the synthetic trace, 
the control law must be very aggressive, sometimes resulting in large queues. As discussed in \S\ref{ss:model1:achievable_bound}, achieving the bound would require a negative sending rate to drain these queues in one time step, which isn't possible.  For the cellular traces, this rarely happens. \ma{can we say somehting about why we didn't run existing congestion controllers on the synthetic trace? for example, if you did and found that they all struggle to keep the queues from blowing up, that's actually interesting because the optimal control law apparently still does a decent job of this} \pg{Synthetic trace went to bandwidths that mahimahi could not support both high and low.} \ma{is the yellow curve a calculation or actual protopcol run on mahimahi for the verizon links? basically do we know that the performance we're talking aout is actually achievable?}\pg{yellow curve is a simulation of the optimal control law. actual achievable performance}

%\pg{Say in practice the performance bound is tight?}

%\pg{Should we say optimizing for E$[\bar{q}]$ and $E[\bar{U}]$ corresponds to $\gamma \to 1$ in the MDP?}

% For each trace, we plot: 1) The performance bound obtained in Theorem~\ref{thm:model1:perfbound}. For cellular traces, we use the distribution of values $\frac{\mu(t)}{\mu(t-1)}$ from the trace as our PDF $f$ to compute the bound;  2) The performance when following the optimal control law obtained in Theorem~\ref{thm:model1:mdp}. We simulate the optimal control law for different values of $C(w, \gamma)$; \cut{The queuing delay and underutilization evolution is governed as per Equations~\eqref{eq:setup:queue_delay_def} and \eqref{eq:setup:undeutilization_def} } 3) Performance of a few existing schemes such as Cubic+Codel~\cite{cubic, CoDel}, XCP~\cite{xcp}, ABC~\cite{abc, goyal2017rethinking}, Sprout~\cite{sprout}, and Copa~\cite{copa}. Here, we emulate the traces using Mahimahi a network emulation tool. For Copa and Sprout, we use the respective author's UDP implementation. For Cubic, we use the linux TCP implementation. For Codel, XCP, and ABC, we use the implementation from ~\cite{abc}. %\pg{include verus?} for this model. There is a fundamental trade-off between underutilization and queuing delay. In particular, we see that achieving very low (close to 0) queuing delay comes at the cost of heavy underutilization and vice-versa.

  \begin{figure}[tb]
 \centering
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortdown_basic.pdf}
        \vspace{-6mm}
        \caption{Verizon Downlink}
        \label{fig:model1:basic:verizon_down}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortup_basic.pdf}
        \vspace{-6mm}
        \caption{Verizon Uplink}
        \label{fig:model1:basic:verizon_up}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_customtrace_basic.pdf}
         \vspace{-6mm}
        \caption{Synthetic Trace}
        \label{fig:model1:basic:generated}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf MIF model performance bound and performance curve for the optimal control law.}}
    \label{fig:model1:basic}
    \vspace{-4mm}
\end{figure} 

%\subsection{Implications for Design of the Control Law}
\smallskip
\noindent
\textbf{Explicit versus implicit feedback:} 
To compute the optimal sending rate, we need the link capacity ($\mu(t-1)$) and queue size ($Q(t-1)$) in the previous time step. Both these quantities are known at the link in time step $t-1$. 
% Therefore, the link itself can compute the optimal sending rate and explicitly communicate it to the sender (via packet headers).
The link can communicate these quantities explicitly to the sender for computing the optimal sending rate. However, explicit feedback is hard to deploy in many scenarios and hasn't seen much adoption in wireless networks~\cite{abc}. Without explicit feedback, the sender needs to infer the link capacity ($\mu(t-1)$) indirectly. This inference is straightforward when there is no link underutilization (the packet arrival rate at the receiver can serve as a measure for the link capacity). However, when the link is underutilized, it can be harder to infer the link capacity at either endpoint~\cite{abc}. 
%For example, if the queue is large enough, the optimal control law requires the sender to stop transmitting entirely until the queue drains in expectation.  \ma{what is the purpose of the last sentence? i don't see the connection to the rest of the paragraph}
% \pg{Do we need this line, the second half is likely wrong? With varying capacity, the link can become frequently underutilized when the link capacity increases, worsening this problem.}
Because implicit feedback introduces uncertainty in the link capacity ($\mu(t)$) at the sender, the resulting performance may be sub-optimal. We see this effect in \Fig{model1:basic}. Explicit schemes like ABC and XCP which compute feedback based on the link capacity outperform end-to-end schemes like Copa and Sprout that infer the link capacity indirectly. 
\ma{i'm ok with this paragraph but it's also ok to cut it. the abc paper already made this point. also the figure isn't very clear about the explcit schemes being that much better}\pg{fine cutting it. I thing a better example would have been to simulate Copa.}

% We hope that our analysis motivates the networking community to change the status-quo and finally adopt explicit feedback.

%Unlike Copa, Sprout, and Cubic+Codel, the sending rate in explict ABC and XCP is based on the link capacity in the previous round. Copa, Sprout, and Cubic+Codel, indeed perform worse than ABC and XCP. 

   \begin{figure}[tb]
 \centering
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortdown_xcpcomp.pdf}
        \vspace{-6mm}
        \caption{Verizon Downlink}
        \label{fig:model1:xcpcomp:verizon_down}
    \end{subfigure}
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortup_xcpcomp.pdf}
        \vspace{-6mm}
        \caption{Verizon Uplink}
        \label{fig:model1:xcpcomp:verizon_up}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_customtrace_xcpcomp.pdf}
         \vspace{-6mm}
        \caption{Synthetic Trace}
        \label{fig:model1:xcpcomp:custom}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf Comparison with XCP/RCP style control law ---} Each XCP curve shows performance for a fixed value of $\alpha$ and variable value of $\beta$ (0 to 10).}
    \label{fig:model1:xcpcomp}
    \vspace{-4mm}
\end{figure} 

\smallskip
\noindent
\textbf{Set sending rate based only on queue size and link capacity:} Some explicit congestion protocols, such as XCP and RCP (for a single sender), set the sending rate according to the following rule\footnote{RCP uses a variant of the rule in which it adjusts the rate in multiplicative  (rather than  additive) increments.}:
\begin{align}
    s(t) = \left( s(t-1) + \alpha \cdot (\mu(t-1) - s(t-1)) - \beta \cdot \frac{Q(t-1)}{T}\right)^+,
\end{align}
where $\alpha$ and $\beta$ are smoothing parameters (typically $< 1$)  that govern stability, how quickly the protocol adapts to spare capacity ($\mu(t-1) - s(t-1))$,
and how aggressively it drains the queue. Unlike our optimal control law, the sending rate in these schemes is dependent on the {\em sending rate} chosen in the previous time step. This does not attempt to keep the relative link load $\rho(t)$ fixed in every time step. Instead, $\rho(t)$ is dependent on congestion control decisions in the previous time steps, and any error in guessing the 
link rate is thus compounded.

Our analysis argues that the performance of such control laws might be sub-optimal on links where the relative uncertainty in link capacity is the same in each time step \ma{on links where the link capacity can vary widely over time (isn't this the more basic point?)}\pg{fine with this, felt the original sentence is more accurate}. To demonstrate this, we simulate an XCP/RCP style control law for various values of $\alpha$ and $\beta$. \Fig{model1:xcpcomp} shows the result for the three traces.  For certain values of $\alpha$ and $\beta$, the performance gets close to the optimal strategy curve. However, for most values the performance deviates from the optimal, and in order to achieve the optimal, we need to tune both $\alpha$ and $\beta$.  For any fixed value of $\alpha$, varying $\beta$ is not optimal across the entire range.



\smallskip
\noindent
\textbf{Do not change the queuing penalty term to adjust the performance trade-off:} Some explicit schemes, such as ABC, follow a different control law of the form:
\begin{align}
    s(t)= \left( \eta \cdot \mu(t-1) - \beta \frac{Q(t-1)}{T}\right)^+,    
\end{align}
where $\eta$ is the target utilization and $\beta$ is a scaling factor for queuing penalty.

This control law is similar to the optimal control law. However, in such control laws the parameter $\eta$ (analogous to $C(w, \gamma)$ in the optimal control law) is incorrectly viewed as the target utilization and is usually set to a value just below one~\cite{abc}. In order to adjust the trade-off between utilization and queuing delay such schemes vary $\beta$. The optimal control law argues that the sender should instead use a fixed value of $\beta = 1$ and vary the parameter $C(w, \gamma)$ (or $\eta$) instead; setting it much less than or greater than one depending on the desired trade-off between queueing delay and underutilization. 

We simulate the ABC style control law for a fixed value of $\eta = 1$ and different values of $\beta$. \Fig{model1:fcvq} shows the result. As expected, the ABC control law deviates from optimal performance, particularly for low values of queueing delay.



   \begin{figure}[tb]
 \centering
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortdown_fcvq.pdf}
        \vspace{-6mm}
        \caption{Verizon Downlink}
        \label{fig:fcvq:verizon_down}
    \end{subfigure}
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortup_fcvq.pdf}
        \vspace{-6mm}
        \caption{Verizon Uplink}
        \label{fig:fcvq:verizon_up}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_customtrace_fcvq.pdf}
         \vspace{-6mm}
        \caption{Synthetic Trace}
        \label{fig:fcvq:generate}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf Comparison with ABC style control law.}}
    \label{fig:model1:fcvq}
    \vspace{-4mm}
\end{figure} 

\if 0
\smallskip
\noindent
\textbf{Achieving the desired performance trade-off:} Depending on the application, a sender might have different requirements for latency and throughput. Given a performance objective ($w$), and a certain discount factor($\gamma$) the sender can calculate $C(w, \gamma)$ in the optimal control law by solving the Bellman Equation. 


Alternatively, \Fig{model1:basic} shows that the performance bound ($g^f$ from \S\ref{ss:model1:performance_bound}) and the optimal control law performance curves are close, and we might be able to use the curve $g^f(\cdot)$ to approximate $C(w, \gamma)$. In particular, we can pick a value of $b$, such that $g^f{'}(x) = -w$ and $x = E[q(t)|\rho(t)=b]$, and correspondingly set $C(w, \gamma)$ to  $b$($=C(w, 0)$) in the optimal control law. \Fig{model1:diff} shows the deviation in performance between this approach and the optimal control law for different values of $b$ and $C(w, \gamma)$. For small values of $b$ and $C(w, \gamma)$, the deviation is small and $b$ is a good approximation for $C(w, \gamma)$. As we increase the value $b$ and $C(w, \gamma)$, the deviation in performance increases. This is because, for higher values of $C(w, \gamma)$, it is more likely that the sender builds an excessive queue ($Q(t-1) > C(w, \gamma) \cdot T \cdot \mu(t-1)$). \pg{This is very weird, Mohammad if possible take a look. The whole business with $\gamma$ makes it a little messy.}\tom{fwiw i'd drop this paragraph and the figure. It doesn't add much that we don't already know - the basic bound is very close in practice.  The divergence of b and C(w, gamma) doesn't seem that important to explain.}\pg{Agreed, it's only going to confuse people}


 \begin{figure}[tb]
 \centering
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortdown_diff.pdf}
        \vspace{-6mm}
        \caption{Verizon Downlink}
        \label{fig:model1:diff:verizon_down}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_verizonLTEshortup_diff.pdf}
        \vspace{-6mm}
        \caption{Verizon Uplink}
        \label{fig:model1:diff:verizon_up}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model1/model1_customtrace_diff.pdf}
         \vspace{-6mm}
        \caption{Synthetic Trace}
        \label{fig:model1:diff:generated}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf Deviation between the performance bound and the optimal control law performance.}}
    \label{fig:model1:diff}
    \vspace{-5mm}
\end{figure} 
\fi 

\smallskip
\noindent
\textbf{Implications for Link Layer Design:} Our analysis also has implications for link layer design (see Appendix~\ref{app:implications_linklayer}). For example, our analysis reveals that variability and uncertainty in link capacity restricts achievable performance. For cellular networks, designing schedulers with a smoother allocation for link capacity can improve performance. Additionally, knowledge about the achievable performance can enable cellular operators to provide guaranteed service level agreements for latency-sensitive applications such as video conferencing.


 \if 0
  \begin{figure}
 \centering
    \begin{subfigure}[tbh]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/tradeoff_Verizon_shortdown.pdf}
         \vspace{-7mm}
        \caption{Trade-off}
        \label{fig:verizon_down:trade-off}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.36\textwidth}
        \includegraphics[width=\textwidth]{images/pdf_Verizon_shortdown.pdf}
        \vspace{-7mm}
        \caption{PDF}
        \label{fig:verizon_down:pdf}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Verizon Downlink}
    \label{fig:verizon_down}
    \vspace{-4mm}
\end{figure}

 \begin{figure}
 \centering
    \begin{subfigure}[tbh]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/tradeoff_Verizon_shortup.pdf}
         \vspace{-7mm}
        \caption{Trade-off}
        \label{fig:verizon_up:trade-off}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.36\textwidth}
        \includegraphics[width=\textwidth]{images/pdf_Verizon_shortup.pdf}
        \vspace{-7mm}
        \caption{PDF}
        \label{fig:verizon_up:pdf}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Verizon Uplink}
    \label{fig:verizon_up}
    \vspace{-4mm}
\end{figure}

\subsection{Applying the model to Cellular traces:}
\Fig{verizon_down} and \Fig{verizon_up} shows the trade-off for two Verizon cellular traces. To generate the trade-off we empirically calculated the PDF $f$ from the trace. The figures also show performance of a number of schemes on these traces in an emulation (using Mahimahi). ABC is an explicit scheme that comes closest to the frontier. \tom{one sentence description of ABC's rule needed here.} In fact, the ABC sender's rate closely corresponds to $\rho(t) = 0.98$ in each round. The ABC point lies close to $C_r = 0.98$ point. Note that, the condition in Eq. ~\ref{eq:boundary_condition} is not met with $C_r = 0.98$, however in both the trace probability $X < \frac{1}{\frac{1}{C_r} + 1}$ or $X < 0.5$is fairly low, as a result excessive queue buildup that hinders the ability to pick a fixed $\rho(t) = C_r$ is rare.

The other congestion control schemes in the figure are purely end-to-end, and as a result the sender might not know $\mu(t-1)$ in round $t$ if the link was underutilized in round $t-1$. As a result, these schemes \textit{will} be unable to pick a sending rate corresponding to a $\rho(t) = C_r$ in such rounds, and the trade-off will thus deviate from the boundary.

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/tradeoff_Verizon_shortup_abc_eta.pdf}
    \vspace{-4mm}
    \caption{\small Verizon Uplink. Performance of ABC with different value of $\eta$. abc\_tcp\_x implies ABC with x/100 as $\eta$. With $\eta = x$, ABC is very similar to a policy $\rho(t) = C_r = x$.}
    \label{fig:verizon_up_eta}
    \vspace{-4.5mm}
 \end{figure}
 
 \Fig{verizon_up_eta} shows performance of ABC with different values of $\eta$. With different value of $\eta$m ABC achieves a different throughput queuing delay trade-off. All the points sit very close to the boundary.
 \fi

==> SIGMETRICS/Model2.tex <==
\section{Incorporating Prediction for Link Capacity}
\label{s:model2}
%\subsection{Model}
\label{ss:model2:model}
%\pg{Merge PMIF into MIF?}
It is natural to ask what if the sender could predict the link capacity with some degree of accuracy? %Can such a prediction improve performance? 
Like the MIF model, does there exist a fundamental performance bound? How can the sender use the prediction and what is the optimal control law? To answer these questions, we will now extend the MIF model to include prediction. We refer to this new model as Prediction-based Multiplicative I.I.D. Factors (PMIF) model. In this model, at the start of every time step, the sender has access to a prediction of the link capacity (e.g., based on past behavior or underlying link information such as signal strength). We denote the link capacity prediction for time step $t$ by $Pred(t-1)$ .

\if 0
\pg{Do we need this? We should just consider this as causal.}
\begin{definition}{\textit{Predictive Congestion Control protocols}---} A predictive congestion control protocol decides the sending rate in time step $t$ based on both observations in earlier time steps along with the prediction for the link capacity. I.e., $s(t)$ is dependent on $\cup_{i=0}^{t-1}\{\mu(i)\}$, $\cup_{i=0}^{t-1}\{U(i)\}$, $\cup_{i=0}^{t-1}\{q(i)\}$, and $Pred(t-1)$.
\end{definition}
\fi 

In the PMIF model, the predicted link capacity can deviate from the true link capacity. We use random variable $X^p$ to represent how far is the prediction relative to the true link capacity. In other words, the random variable $X^p$ is a measure of uncertainty in the true link capacity given the prediction. %Moreover, we assume this uncertainity for each round is the same.
Formally, the uncertainty in the link capacity is governed by,
\begin{equation}
    \mu(t) = Pred(t - 1) \cdot X_{t}^p,
    \label{eq:model2:model}
\end{equation}
where  $X_{i}^p$ is an I.I.D random variable with $f^p(\cdot)$ as its probability density function (PDF) and $P(X_{i}^p <= 0) = 0$. %The uncertainty is link capacity relative to its expected value has the same characteristics in every time step.%We assume $X_{i}^t$ is independent of $s(t), Q(t-1), \mu(t-1), Pred(t-1)$.

%As before, we derive a performance bound between $E[\bar{q}(t)]$ and $E[\bar{U}(t)]$ (\S\ref{ss:model2:performance_bound}). We use this analysis to draw insights about  the optimal controller (\S\ref{ss:model2:achievable_bound}). Next, we a MDP (\S\ref{ss:model2:mdp}). We sketch some implications of our analysis and validate our findings (\S\ref{ss:model2:implications}). 

\pg{As before, we derive a performance bound between $E[\bar{q}(t)]$ and $E[\bar{U}(t)]$ (\S\ref{ss:model2:performance_bound}). We use this analysis to draw insights about the optimal controller and derive the optimal control by posing the problem as a particular MDP (\S\ref{ss:model2:mdp}). We sketch some implications of our analysis and validate our findings (\S\ref{ss:model2:implications}).}

Note that, we do not attempt to come up with a predictor ourselves; rather, we only analyse the impact of prediction error on the design of congestion control for time-varying links.

\subsection{Performance Bound}
\label{ss:model2:performance_bound}

\begin{corollary}

In the PMIF model, for any causal congestion control protocol, for any $t \in \mathbb{N}$, the point ($E[\bar{q}(t)]$, $E[\bar{U}(t)]$) always lies in a convex set $\mathbb{C}^{f^p} \triangleq \{(x,y) | y>=g^{f^p}(x)\}$, where $g^{f^p}(\cdot)$ is defined by Eq.~\eqref{eq:model1:thm:perfbound}.
\label{cor:model2:perfbound}
\end{corollary} 

The performance bound is dependent on the characteristics of the random variable $X^p$ and consequently the accuracy of prediction. The better the prediction, the better the performance bound.

\begin{proof}
To prove this corollary, we will use the techniques from the proof of Theorem ~\ref{thm:model1:perfbound}. Using $\mu(t) = Pred(t-1) \cdot X^p_t$, we can rewrite the equation describing underutilization and queuing delay as follows,

\begin{align}
    q(t) &= T \cdot \left(\frac{\frac{Q(t-1)}{T} + s(t)}{Pred(t - 1) \cdot X_{t}^p} - 1 \right)^+, &  U(t) = \left( 1 - \frac{\frac{Q(t-1)}{T} + s(t)}{Pred(t - 1) \cdot X_{t}^p}\right)^+.\nonumber\\
    \label{eq:prediction_system}
\end{align}

Similar to $\rho(t)$ from Eq.~\eqref{eq:model1:proof_perfbound:rt}, we define a new quantity $\rho^p(t)$ as follows,
\begin{align}
    \rho^p(t) &=  \frac{\frac{Q(t-1)}{T} + s(t)}{Pred(t - 1)}.
    \label{eq:prediction_rt}
\end{align}

Intuitively, $\rho^p(t)$ can be thought of as the load on link in time step $t$ relative to the prediction of the link capacity ($Pred(t-1)$). We can rewrite $q(t)$ and $U(t)$ in terms of $\rho^p(t)$,

\begin{align}
    q(t) &= T \cdot \left(\frac{\rho^p(t)}{X_{t}^p} - 1 \right)^+, &U(t) &= \left(1 - \frac{\rho^p(t)}{X_{t}^p}\right)^+.
    \label{eq:prediction_qU_rt}
\end{align}

Notice that the equation above is analogous to Eq.~\eqref{eq:model1:proof_perfbound:qU_rt}. Thus, we can apply the same techniques as in the proof for Theorem ~\ref{thm:model1:perfbound} to show that the point $(E[q(t)|\rho^p(t)=b], E[U(t)|\rho^p(t)=b])$ lies on the curve $g^{f^p}(\cdot)$. Both the points $(E[q(t)], E[U(t)])$ and $(E[\bar{q}(t)], E[\bar{U}(t)])$ lie in the convex set $\mathbb{C}^{f^p}$. %Corollary proved.
\end{proof}

\if 0
\subsection{Is the Performance Bound Achievable?}
\label{ss:model2:achievable_bound}

The analysis in the previous section shows us that we can achieve a particular point $(x, g^{f^p}(x))$ on the performance bound %where $x = (T \cdot \int_{0}^{C}\left(\frac{C}{a} - 1 \right) \cdot f^p(a) \cdot da)$ 
by following a strategy of the form,
\begin{align}
    \rho^p(t) &= C^p, &
    s(t) &= C^p \cdot Pred(t-1) - \frac{Q(t-1)}{T}, & \forall t \in \mathbb{N},
    \label{eq:model2:ab_guess_control}
\end{align}
where $E[q(t)|\rho^p(t)=C^p] = x$.%$C \in R+$. 

The key is keeping the link load relative to the prediction of the link capacity the same in every time step, regardless of the state of the system. Again, following this strategy might not be possible for all values of $C^p$. In the event of excessive queuing ($Q(t-1) > T \cdot C^p \cdot Pred(t-1)$), for $\rho^p(t)= C^p$, the sender needs to pick a negative value for $s(t)$ (from Eq. \eqref{eq:prediction_rt}) which is not possible.% In such a scenario, the performance point ($E(\bar{q}(t)$, $E(\bar{U}(t)$) might not be on the boundary of set $\mathbb{C}^f$. 
We will now establish the necessary conditions under which the sender can follow the strategy $\rho^p(t) = C^p$ exactly. %Let $X^{p}_{min}$ be the minimum value of $X$ given the PDF $f$ ($P(X^{p}<X^{p}_{min}) = 0$). 

\begin{proposition}
In the PMIF model, it is possible to follow the strategy $\rho^{p}(t) = C^p$, $\forall t \in \mathbb{N}$ iff
\begin{align}
    C^p \cdot \left(1 - \frac{Pred(t)}{Pred(t-1)}\right) &\leq  X^p_{min}, & \forall t \in \mathbb{N},
    \label{eq:prop:model2:achievable_bound}
\end{align}
\label{prop:model2:achievable_bound}
\end{proposition} 
where $X^{p}_{min}$ is the minimum value of $X^p$ ($P(X^{p}<X^{p}_{min}) = 0$)
\begin{proof}
 Please see Appendix~\ref{app:model2:achievable bound} for the proof.
\end{proof}

Interestingly, this condition depends on the ratio of $Pred(t)$ and $Pred(t-1)$. 
The lower the ratio, the more stringent the constraint on $C^p$. 
If the prediction for the link capacity decreases, then it is more likely for the link capacity to decrease enough for the sender to build up an excessive queue. Again, this condition establishes that the performance bound might not be tight. %For any $f^p(\cdot)$, only the points $\{x, g^{f^p}(x)\}$ where $E[q(t)|\rho^p(t)=C^p] = x$ and $C^p$ meets the condition above are achievable.
%\tom{advise rewriting the above text a bit if possible - its just a bit weird to say it like this.  The issue is the link capacity variation from one time step to the next. on the other hand you depend on it below.}
%\pg{I thought about it, I was not be able to come up with much. I will rewrite it if I come up something better.}

\ma{I suggest cutting this subsection entirely. It's pretty repetitive with the previous model, and the result is a bit weird. Earlier the condition was crisply defined in terms of the input distributions of the problem. Here it depends on a time-varying ratio of the predictions. It doesn't seem that useful. You could probably improve it by replacing the time-varying ratio with the max of the ratio over time. But still think it's better to just cut it and come to the optimal control law more quickly. You could start the next section simply as follows}

\fi


%\subsection{\todo{Optimal Control law, Feedback NEEDED}}
\subsection{Optimal Control Law}
\label{ss:model2:mdp}
The analysis in the previous section shows us that we can achieve a particular point $(x, g^{f^p}(x))$ on the performance bound by following a strategy of the form,
\begin{align}
    \rho^p(t) &= C^p, &
    s(t) &= C^p \cdot Pred(t-1) - \frac{Q(t-1)}{T}, & \forall t \in \mathbb{N},
    \label{eq:model2:ab_guess_control}
\end{align}
where $E[q(t)|\rho^p(t)=C^p] = x$. The key is keeping the link load relative to the prediction of the link capacity the same in every time step, regardless of the state of the system. However, similar to \S\ref{ss:model1:achievable_bound}, following this strategy might not be possible for all values of $C^p$. In the event of excessive queuing ($Q(t-1) > T \cdot C^p \cdot Pred(t-1)$), for $\rho^p(t)= C^p$, the sender needs to pick a negative value for $s(t)$ (from Eq. \eqref{eq:prediction_rt}) which is not possible. Is simply following $s(t) = (C^p \cdot Pred(t-1) - \frac{Q(t-1)}{T})^+$ optimal in just situations?


%\pg{is it even needed? We should only include math for which can de experiments}
%What happens when the above condition is not met? Will the following variant of the strategy in Proposition~\ref{prop:model2:achievable_bound} -- $\rho^p(t) = max(C^p, \frac{Q(t-1)}{Pred(t-1) \cdot T})$ or $s(t) = (C^p \cdot Pred(t-1) - \frac{Q(t-1)}{T})^+$ -- be optimal? 

Similar to the MIF model, we can formulate the congestion control task as a MDP and show that the above control law is optimal. The key change in the MDP from the MIF model is that the state in time step $t$ is now given by ($q(t-1), \mu(t-1), Pred(t-1)$). \pg{We find that the optimal control law for the MDP depends on the dynamics of the predictions. 
At a high level, the dynamics of the prediction affect how the link capacity varies from one time step to the next and consequently the dynamics of (excessive) queue build up.
Here, we only derive the exact optimal control law for a simple model governing the evolution of $Pred$. In this model the evolution of $Pred$ is analogous to evolution of $\mu$ from the MIF model. Formally,}
%Additionally, we must assume some dynamics for the predictions in the MDP. This dynamics impacts the control law \ma{This is the tricky sentence. How? is it relevant to constants or the form of the controller. Right now $f^{pred}$ doesnt seem to be showing up at all in the result. I am assuming it impacts the constant.}. For this MDP, we use a simple model governing the evolution of $Pred$,
\begin{align}
    Pred(t) = Pred(t-1) \cdot X^{pred}_{t},    
\end{align}
where  $X_{i}^{pred}$ is an I.I.D random variable with $f^{pred}$ is its probability density function (PDF) and $P(X_{i}^{pred} \leq 0) = 0$. Other state transitions are governed by,
\begin{align}
    \mu(t)&=\mu(t-1)\cdot X^p_t \quad \text{(per the PMIF model)}, \nonumber\\
    q(t)&=T\cdot(\rho^p(t)/X^p_t-1)^+ \quad \text{(per Eq.~\eqref{eq:prediction_qU_rt})}, \nonumber
\end{align}


The goal of the agent is to minimize the objective function ($J(\cdot)$ from Eq.~\eqref{eq:model1:mdp:objective}) over all policies ($\pi$).

\if 0
\begin{align}
     J^p(\pi^p) = E\left[\sum_{t=1}^{\infty}\gamma^{t-1} \Big( w \cdot q(t) + U(t)] \Big)\right], 
\end{align}
where $\gamma \in (0,1)$ is the discount factor. 
\fi

\begin{corollary}
    In the MDP defined above, the optimal control policy that minimizes $J(\pi)$ takes the form:  
    \begin{align}
        s(t) = \left( C^p(w, \gamma) \cdot Pred(t-1) - \frac{Q(t-1)}{T} \right)^+,  
        \label{eq:cor:model2:mdp}
    \end{align}
where $C^p(w,\gamma)$ is a constant. 
    \label{cor:model2:mdp}
\end{corollary}
\begin{proof}
Please see Appendix~\ref{app:model2:cor_mdp}
\end{proof}


\if 0
In particular, our goal is to find a causal congestion control strategy, s.t., we minimize the value of the following objective function,
\begin{align}
 \sum_{i=t}^{n}\gamma^{i-t} \Big( w \cdot E[q(i)] + E[U(i)] \Big), && \forall t \leq n,
\end{align}
where $\gamma$ is the discount factor and $\gamma \in (0,1)$.

In the previous subsection, we saw that the condition for whether a point on the performance bound is achievable or not depends on $\frac{Pred(t)}{Pred(t-1)}$. The exact dynamics of $Pred$ can impact the optimal control law. For the MDP, we use a simple model governing the evolution of $Pred$,
\begin{align}
    Pred(t) = Pred(t-1) \cdot X^{pred}_{t},    
\end{align}
where  $X_{i}^{pred}$ is an I.I.D random variable with $f^{pred}$ as its probability density function (PDF) and $P(X_{i}^{pred} <= 0) = 0$.

We will now write the Bellman Equation governing this optimization problem. Where $V_{t-1}(\cdot)$\cut{$(\frac{Q(t-1)}{Pred(t-1)})$}  is the value function at time step $t-1$

\begin{align}
    V_{t-1}(\frac{Q(t-1)}{Pred(t-1)}) &= \min_{\rho^p(t) \geq \frac{Q(t-1)}{T \cdot Pred(t-1)}}  \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot E[V_{t}(\frac{Q(t)}{Pred(t)})]\Bigg), & \forall t \leq n.\nonumber\\
   V_{t}(\frac{Q(t)}{Pred(t)}) &= 0, & t=n.
\end{align}

\if 0
\begin{align}
    V_{t-1}(\frac{Q(t-1)}{Pred(t-1)}) &= \min_{s(t) \geq 0} \Bigg( w \cdot E[q(t)] + E[U(t)] + \gamma \cdot \int_{0}^{\infty}f^p(a) \cdot V_{t}(\frac{Q(t)}{Pred(t)}) \cdot da\Bigg) \nonumber &, \forall t < n\\
   V_{t}(Q(t),\mu(t)) &= 0 &, t=n
\end{align}
\fi


Similar to (\S\ref{ss:model1:mdp}), we can describe the function $V_{t-1}$ using only $\frac{Q(t-1)}{Pred(t-1)}$.
This is beacuse, in the equation above, the first two terms on the right hand side ($E[U(t)]$ and $E[q(t)]$) depend only on the value of $\rho^p(t)$. Since $\frac{Q(t)}{Pred(t)}$ (= $ T \cdot (\frac{\rho^p(t)}{X^p_t} - 1)^+  \cdot \frac{X^p_t}{X^{pred}_t}$) only depends on $\rho^p(t)$, this implies that if $V_{t}$ is only a function of $\frac{Q(t)}{Pred(t)}$, then $V_{t-1}$ is also only a function of $\frac{Q(t-1)}{Pred(t-1)}$.  Rewriting,  


\begin{align}
    V_{t-1}(\frac{Q(t-1)}{Pred(t-1)}) = \min_{\rho^p(t) \geq \frac{Q(t-1)}{T \cdot Pred(t-1)}} &\Bigg( w \cdot E[q(t)] + E[U(t)]\nonumber\\ &+ \gamma \cdot \int_{0}^{\infty}\int_{0}^{\infty}f^p(a) \cdot f^{pred}(b) \cdot V_{t}(T \cdot (\frac{\rho^p(t)}{a} - 1)^+ \cdot \frac{a}{b}) \cdot da \cdot db\Bigg)\nonumber &, \forall t \leq n\nonumber\\
    % V_{t-1}^1(\frac{q(t-1)}{T}) &= \min_{r(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
    \label{eq:model2:v_def}
\end{align}

To help our analysis, we define a new helper function  $V_{t}^2(\rho^p(t))$ as follows,
\begin{align}
    V_{t-1}(\frac{Q(t-1)}{Pred(t-1)}) &= \min_{\rho^p(t) \geq \frac{Q(t-1)}{T \cdot Pred(t-1)}} (V_{t}^2(\rho^p(t))).\nonumber\\
    %V_{t}^2(r(t)) &= \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    %&+ \int_{0}^{\infty}f(a) \cdot V_{t-1}^1((\frac{r(t)}{a} - 1)^+) \cdot da\Bigg)\nonumber &, \forall t<n\nonumber\\
\end{align}

\begin{lemma}
$\forall t \leq n$, both $V_{t-1}(\cdot)$ and $V_{t}^2(\cdot)$ are convex.
\label{lemma:model2:mdp_convex}
\end{lemma}
The proof for this lemma is almost identical to proof of Lemma~\ref{lemma:model1:mdp_convex}, except we need to redefine $h_a(\cdot)$ from Sub lemma~\ref{sublemma:model1_helper} as follows.
\begin{align}
    h_{a,b}(x) = T \cdot (\frac{x}{a}-1)^+ \cdot \frac{a}{b}
\end{align}


This Lemma establishes that the best strategy in any given time step $t$ is of the following form,
\begin{align}
    \rho^p(t) &= max(C^p(w,t), \frac{Q(t-1)}{T \cdot Pred(t-1)}), & s(t) = \left(C^p(w, t) \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)^+,
\end{align}
where the minimum value of $V^2_{t}(\cdot)$ occurs at $r(t) = C^p(w, t)$ or $V_{t-1}(0) = V^2_{t}(C^p(w, t))$. We can calculate the exact value of $C^p(w, t)$ by solving the Bellman equation.% starting from round $n$ and working backwards.

%This Lemma establishes that the best strategy in any given round $t$ is of the following form: $s(t) = \left(C(w, t) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)^+$ or $r(t) = max(C(w,t), \frac{q(t-1)}{T})$ where the minimum value of $V^2_{t}$ occurs at $r(t) = C(w, t)$ or $V_{t-1}(0) = V^2_{t}(C(w, t))$.  We can calculate the exact value of $C(w, t)$ by solving the Bellman equation starting from round $n$ and working backwards.

\if 0
The optimal strategy is of the form. (\todo{prove Convexity of V just as before}). 
\begin{align*}
    s(t) = max\left(0, C(\cup_{i=t-1}^{n} \{Pred(i)\}) \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

Note that this is assuming $Pred$ as constant (\pg{is this a good assumption, i wonder if I should also impose some rules on evolution of $pred$, maybe for something like $pred(t) = pred(t-1) \cdot X$ we can show $V$ as a function of $\frac{Q(t)}{Pred(t)}$. I think with this we will get a clean strategy of the form $s(t) = mac(0, C \cdot Pred(t-1) - \frac{Q(t-1)}{T}$.}


Consequently, I believe the following simpler strategy will achieve performance close to the bound.

\begin{align*}
    s(t) = max\left(0, C \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}
\fi

Next, we consider this MDP over infinite horizon.


\begin{conjecture}
    As $n \to \infty$, $V_{t-1}(x) \to V_{0}(x)$ and $V_{t}^2(x) \to V_{1}^2(x), \forall t << n$ and $x \in \mathbb{R}^+$.
    \label{conj:model2:value_function}
\end{conjecture}
\pg{can we prove the conjecture if not give some intuition behind why we think the conjecture is true.}

\begin{corollary}
    In the model~\S\ref{ss:model2:model}, for the MDP~\S\ref{ss:model2:mdp}, if Conjecture~\ref{conj:model2:value_function} holds, then $n \to \infty \forall t << n$, the following causal congestion control protocol is optimal. 
    \begin{align}
        s(t) = \left( C^p(w) \cdot Pred(t-1) - \frac{Q(t-1)}{T} \right)^+,  
        \label{eq:cor:model2:mdp}
    \end{align}
    \label{cor:model2:mdp}
\end{corollary}
where $V_{0}(0) = V^2_{1}(C^p(w))$.

Proof: Directly follows from Conjecture~\ref{conj:model2:value_function}.

This corollary establishes that for all rounds, the sender should try to keep the link load relative to the prediction constant ($\rho^p(t) = C^p(w)$). In the event of excessive queuing ($Q(t-1) > T \cdot C^p(w) \cdot Pred(t-1))$), the sender should pick the minimum possible value for relative link load ($\rho^p(t) = \frac{Q(t-1)}{T \cdot Pred(t-1)}$ or $s(t) = 0$).


%\pg{Give mathematical intuition and implication everywhere.}

%\tom{is there a version of figure 7 that you could put here?  That is, use ML to predict the next rate from the previous rates, with no restrictions on the model, and pick some fixed $C_r$.  Overfitting is an issue so only do the training on the first half of the trace, and only report results on the second half. Does this outperform the previously optimal line based on an assumption of unpredictability in the subsequent rate?  Or would that graph look exactly the same as Figure 7?}
\fi

\subsection{Implications and Validation}
\label{ss:model2:implications}

%\textbf{Good prediction can improve performance substantially:} 
\pg{To demonstrate that good prediction can improve performance substantially this model, we use the traces from} \S\ref{ss:model1:implications}. At the start of each time step $t$, we synthetically supply a prediction ($Pred(t-1)$) to the sender. To demonstrate improvements over the optimal control law (without prediction) from the MIF model, we intentionally pick a prediction with good accuracy ($X^p \sim U (0.8, 1.2)$) such that for each trace $g^{f^p}$ is better than $g^f$. Using $X^p$ and $\mu(t)$, we sample the value for $Pred(t-1)$ with Eq.~\eqref{eq:model2:model} as follows:
\begin{align}
    Pred(t-1) = \frac{\mu(t)}{X^p}.
\end{align}


\Fig{model2:basic} shows the performance bound ($g^{f^p}(\cdot)$) obtained in Corollary~\ref{cor:model2:perfbound}. The figure also shows the performance curve when following the optimal control law from Corollary~\ref{cor:model2:mdp} for different values of $C^p(w, \gamma)$. We also include the performance bound ($g^f(\cdot)$) and the performance curve of the optimal control law based on the MIF model. Indeed, the optimal control law with prediction  outperforms that based on the MIF model.
Additionally, the optimal control law achieves performance close to the performance bound. 

\pg{This result shows that that improving link rate prediction could provide large performance gains. Besides better statistical modeling, it is likely that the largest gains could result from better signals from the link layer and  wireless schedulers~\cite{pbe_cc, xie2015pistream}.} \pg{citation is meh}
%\pg{I cut some text here (in comments).}%We can use $g^{f^p}(\cdot)$ to calculate an approximate value for $C^p(w, \gamma)$ in the optimal control law. To achieve a desired trade-off $w$, we can use  $g^{f^p}(\cdot)$ to calculate a $b$ such that $g^{f^p}{'}(x) = -w$ ($x$ is from Eq.~\eqref{eq:model1:thm:perfbound}) and correspondingly set $C^p(w, \gamma)$ to $b$(=$C^p(w, 0)$) in the optimal control law.


   \begin{figure}[tb]
 \centering
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model2/model2_verizonshortdown.pdf}
        \vspace{-6mm}
        \caption{Verizon Downlink}
        \label{fig:model2:basic:verizon_down}
    \end{subfigure}
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model2/model2_verizonshortup.pdf}
        \vspace{-6mm}
        \caption{Verizon Uplink}
        \label{fig:model2:basic:verizon_up}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model2/model2_customtrace.pdf}
         \vspace{-6mm}
        \caption{Synthetic Trace(MIF model)}
        \label{fig:model2:basic:custom}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf Impact of incorporating prediction ---} Incorporating prediction can substantially improve performance.}
    \label{fig:model2:basic}
    \vspace{-4mm}
\end{figure} 

% For the cellular traces, we only have data for the link capacity. Given that we don't have any visibility into the specifics of the link layer design or the underlying link information governing the link capacity, 
\if 0
\smallskip
\noindent
\textbf{Prediction based only on past link capacity:} For the traces from \S\ref{ss:model1:implications}, can we predict the current link capacity based on recent observations of the link capacity? For example, we may not have access to physical layer information such as signal strength. To this end, we built a simple predictor based on the link capacity over the last five time steps. Formally, $Pred(t-1) (= \sum_{i = 1}^{5} w_i \cdot \mu(t-i))$ is a weighted average of the link capacity in the time steps $t-5$ to $t-1$. Given a particular set of weights, we can empirically compute the random variable $X^p$ associated with this predictor using the trace.\footnote{We use the distribution of $\frac{\mu(t)}{Pred(t-1)}$ from the trace as the PDF for $X^p$ ($f^p$).} We use a simple heuristic, and pick the weights with the minimum value of standard deviation for the random variable $log(X^p)$ for this predictor.
%To set the weights: for different weights we compute the random variable $X^{p}$ given the trace, and pick weights with the minimum standard deviation for the random variable $log(X^p)$.
\Fig{model2:sep} shows the performance curve for the PMIF model optimal control law with this predictor -- it does not provide any benefit relative to the simpler MIF model. 
% We find that the performance with this predictor does not provide any improvements over the optimal control law from the MIF model. To build a better predictor for such cellular links, we might need additional link layer information. 
\ma{Seems weak. So what that a moving average predictor didn't work? Maybe the model sucks, or maybe there isn't enough correlation (but you can't conclude that). I'd cut this. Instead, end 6.3 with a sentence like: This result shows that that improving link rate prediction could provide large performance gains. Besides better statistical modeling, is likely that the largest gains could result from better signals from the link layer and  wireless schedulers. (Cite any work that exists on this) }

% We hope that our analysis motivates researchers to build better predictors for link capacity and improve congestion control performance.


   \begin{figure}[tb]
 \centering
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model2/model2_verizonshortdown_sep.pdf}
        \vspace{-6mm}
        \caption{Verizon Downlink}
        \label{fig:model2:sep:verizon_down}
    \end{subfigure}
     \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model2/model2_verizonshortup_sep.pdf}
        \vspace{-6mm}
        \caption{Verizon Uplink}
        \label{fig:model2:sep:verizon_up}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \includegraphics[width=\textwidth]{SIGMETRICS/images/model2/model2_customtrace_sep.pdf}
         \vspace{-6mm}
        \caption{Synthetic Trace(MIF model)}
        \label{fig:model2:sep:custom}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf Simple predictor based only on past link capacity observations---} $Pred(t-1) = \sum_{i = 1}^{5} w_i \cdot \mu(t-i)$.}
    \label{fig:model2:sep}
    \vspace{-4mm}
\end{figure} 
\fi

==> SIGMETRICS/introduction.tex <==
\section{Introduction}
\label{s:intro}
Recently, several new congestion control protocols have been proposed for improving performance on time-varying wireless links such as Cellular or WiFi ~\cite{abc, sprout, verus, copa, pcc}. Broadly, the goal of any such protocol is to reduce queue at the bottleneck link while maintaining a high level of link utilization or throughput. 
However, achieving both low queuing and high utilization is challenging. Unlike wired links, wireless links can exhibit variations in the link capacity over time. Congestion control protocols adjust the sending rate based on feedback signals from the network. The feedback is typically delayed by a round trip time (RTT), the capacity of the link and the appropriate sending rate can change significantly within a RTT causing underutilization or queuing.

The feedback delay creates an uncertainty about the current link capacity at the sender for deciding the sending rate. The design of existing congestion control schemes is by and large agnostic to the characteristics of this uncertainty. We find that their performance is sub optimal and there is significant room for improvement. Understanding this uncertainty, can help us improve performance. In this work, we show that the uncertainty in link capacity presents a \textit{fundamental} trade-off in performance (between underutilization and delay) for congestion control schemes. This trade-off is not because the link capacity is changing but rather because the sender doesn't know what the current link capacity is deterministically. Moreover, the nature of the uncertainty has important implications for design of the congestion control loop itself.
%where the sender picks the sending rate based on observations in the past (i.e., the sender is not predicting the link capacity in future).

To capture the uncertainity in link capacity, we use three simple discrete-time markov chain models for the link capacity with increasing complexity. For each model, we derive a bound on the best possible performance congestion control protocols can achieve in expectation (Theorem~\ref{thm:model1:perfbound}, Corollary~\ref{cor:model2:perfbound} and \ref{cor:model3:perfbound}).\footnote{We chose a linear combination of expected queuing delay and expected link underutilization as our performance metric.} This bound is a function of the uncertainity in link capacity at the sender, the more uncertain the link is the worse the bound. This analysis also provides us insights and a rough sketch of the optimal congestion control loop. Next, for each model, we pose the problem of selecting the sending rate as markov decision process and derive the optimal congestion control loop (Theorem~\ref{thm:model1:mdp}, Corollary~\ref{cor:model2:mdp} and \ref{cor:model3:mdp}). Again, the optimal control loop in each model is governed by the nature of uncertainty in link capacity and differs from control loops used by existing schemes.

Note that the real wireless links need not follow the models we use. Our goal is not to construct perfect models for link capacity variation. Instead, we focus on these models to draw insights about the optimal congestion control loop and show that these insights can actually lead to performance improvements. We use real cellular traces to validate the insights from our analysis. 

\pg{Should we include diagrams of the markov chain for the three models?}

\textbf{Model 1: Restricted markov chain (\S\ref{s:model1}):}
In this model, the link capacity at time $t$ ($\mu(t)$) is dependent on the capacity in the previous RTT ($\mu(t-1)$) as follows,
\begin{align}
    \mu(t) = \mu(t-1) \cdot X_t
\end{align}
where $X_t$ are I.I.D random variables. In this model, the relative uncertainity in relative link capacity in same in every round and is governed by characteristics of $X$. %This model is relatively easier to understand and analyse. %We use insights from analysis of this model for other more complex models.
Under assumptions of the model, the optimal control loop for a single flow is of the simple form,
\begin{align}
    s(t) = (C \cdot \mu(t-1) - \frac{Q(t-1)}{T})^+    
\end{align}
where $T$ is the base RTT, $Q(t)$ is the queue size. $C$ is a positive constant that depends on the performance objective and characteristics of $X$. In our evaluation over real cellular traces, the optimal control loop outperforms existing schemes.

\textbf{Model 2: Prediction for link capacity (\S\ref{s:model2}):}
In this model, we consider scenarios where the sender has access to a prediction ($Pred(t-1)$) about the current link capacity ($\mu(t)$). We assume that the prediction in not perfect and has inaccuracies. The uncertainty in link capacity at the sender is governed by,
\begin{align}
    \mu(t) = Pred(t-1) \cdot X^p_t
\end{align}
where $X^p_t$ are I.I.D random variables.
The optimal control loop in this model is of the form,
\begin{align}
    s(t) = (C \cdot Pred(t-1) - \frac{Q(t-1)}{T})^+    
\end{align}
where $C$ is a positive constant that depends on the performance objective and characteristics of $X^p$. We find that a good predictor for link capacity can substantially improve performance on our cellular traces.

\textbf{Model 3: Generic markov chain (\S\ref{s:model3}):} In this model, we relax the constraints in Model 1. We assume a generic markov chain for how the aggregate link state governing the link capacity (depicted by $S(t)$) evolves. In this model, the uncertainity in link capacity is governed by,
\begin{align}
    \mu(t) &= Y_t^{S(t-1)}\nonumber\\
    S(t) &= Z_{t}^{S(t-1)}
\end{align}
where $Y_t^{S(t-1)}$ and $Z_t^{S(t-1)}$ are I.I.D random variables. 
The optimal control loop is of the form,
\begin{align}
    s(t) = (C^{S(t-1)} \cdot \mu(t-1) - \frac{Q(t-1)}{T})^+    
\end{align}
where $\textbf{S}$ represents the space of all possible states $S(t)$, and, $C^{k}, \forall k \in \textbf{S}$ is a positive constant that depends on the random variables $\cup_{k \in S}\{Y^k\}$ and $\cup_{k \in S}\{Z^k\}$. On cellular traces, this control loop improves performance over the (simpler) optimal control loop for Model 1.

The form of the optimal control loop in all the models presents a strong case for explicit congestion control~\cite{abc, xcp, rcp}. In particular, the bottleneck wireless router/cellular base station has direct access to the underlying information such as link capacity($\mu$), queue size($Q)$, and link state ($S$), and can thus compute the optimal sending rate (for all models) and communicate it explicitly to the sender. For end-to-end schemes~\cite{verus, sprout, copa, CoDel}, the sender might need to infer such link information indirectly. Such inference might have errors~\cite{abc}, and consequently sub-optimal performance.
%\pg{Our analysis presents a strong case of explicit congestion control where the wireless router/cellular base station explicitly signals the sending rate to the end-point based characteristics of the potential uncertainity.}

While we only analyze these three models, our techniques are general and could potentially be applied to other markovian models of link capacity variation and for different performance objectives than the ones we use. 

\pg{Implications for scheduler design, application to datacenter stuff where the uncertainity is because of changing competing users?} 

\pg{Do we need a backgroun/motivation section?}

%where $Pred(t-1)$ is the link capacity prediction for round $t$. This is a model which assumes that the protocol makes a prediction for the next round and the link capacity varies from the prediction in an uncertain way. The equations governing the system are very similar to the one in Model 1. We prove a bound on performance similar to model 1, depends only on $f^p$ (PDF of $X^p$), see \S\ref{s:model2}.

%Based on the model, we either consider both causal or predictive class of congestion control protocols. In causal protocols, the sender picks the sending rate based solely on observations in the past. In predictive protocols, the sender also uses a prediction about the current link capacity. For such protocols, the inaccuracy in the prediction governs the achievable performance and the optimal congestion control loop. 


\if 0
%We find that for the first two models that we consider, the optimal congestion control loop has a simple closed form. For the last model, the optimal congestion control 

%Intuitively, the bound on trade-off is fundamental because the sender adjusts its rate based on observations such as queuing delay, link capacity, etc. in the past (delayed by the propagation delay). By the time sender adjusts its rate, the link conditions might have changed. The randomness of the change in link capacity can cause the sender to either under-utilize the link (if the link capacity increased) or build up excessive queuing. 


%We begin by modelling the randomness on variations in link capacity using a discrete-time stochastic model. Under this model, the link capacity at a time step $t$ is a random variable dependent on the link capacity at time step $t-1$. In particular, the randomness in the link capacity in any given time step is similar. With this model, we prove a bound on the expected underutilization-expected queuing delay trade-off. Any causal congestion control protocol will achieve the same or worse trade-off than this bound. We also provide close to optimal congestion control strategies that either achieve the trade-off bound or are very close. The bound itself is a function of the randomness in capacity variations. On increasing the randomness, the bound worsens.  


%We then expand this model to incorporate non-causal congestion control protocols with future predictions of link capacity, and show that the trade-off bound improves as the prediction gets better. We also expand our link variation model to a generic markov chain model.


\subsection{What results/theorems have we proved?}
We present analysis on performance of congestion control protocols on links with time-varying capacity. Because of the uncertainty in the link capacity, any protocol can only achieve a certain link utilization queuing delay trade-off. the The analysis reveals a bound on the performance a protocol can achieve and also reveals the optimal congestion control protocol. We model the link capacity ($\mu(t)$) as discrete time stochastic process. We consider three stochastic processes.

\textbf{Model 1: Causal congestion control protocols, uncertainty in link capacity is similar in each time step.}
\begin{align*}
    \mu(t) = \mu(t-1) \cdot X
\end{align*}
where $X$ is a random variable with PDF $f$. A key characteristic of this model is the uncertainty in link capacity in every time-step is similar (characterized by $f$). This assumption makes the model easy to analyze and provides a good starting point. We prove a lower bound on the performance in terms of expected queuing delay and link underutilization using stochastic analysis (see \S\ref{ss:model1:performance_bound}) for causal congestion control protocols. 

\textit{MDP.} To find the optimal congestion control strategy we pose the problem as a MDP with achieving high utilization and low queuing delay as the objective function. Using Bellman equations to describe the system, we can find the optimal strategy (see \S\ref{ss:conjecture}). Interestingly, we find that for infinitely long runtime, the optimal strategy is very simple

\begin{align*}
    s(t) = max\left(0, C \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

\textcolor{red}{Not done: Close the gap in the proof above.} We need to make this statement precise.

\textcolor{red}{Not done: Generalizing the MDP.} We can generalize the objective function in the MDP. I think the result holds as long as the objective function is just a function of $r(t)$ and is convex in $r(t)$.

\textit{Application to real traces.} We applied the model on a few cellular traces. The bound on performance on these traces seem real, existing congestion control schemes achieve performance worse than the predicted bound. We also ran the above optimal strategy and found the performance is actually very close to the predicted bound.

\textbf{Model 2: Predictive congestion control protocols,  uncertainty in link capacity is similar in each time step.}
\begin{align*}
    \mu(t) = Pred(t-1) \cdot X^p
\end{align*}
where $Pred(t-1)$ is the link capacity prediction for round $t$. This is a model which assumes that the protocol makes a prediction for the next round and the link capacity varies from the prediction in an uncertain way. The equations governing the system are very similar to the one in Model 1. We prove a bound on performance similar to model 1, depends only on $f^p$ (PDF of $X^p$), see \S\ref{s:model2}.  

\textcolor{red}{Not done: Posing it as a MDP} Posing the problem as a MDP and using bellman equations. I believe this will not reveal a simple optimal strategy as in Model 1. My guess is a strategy of the following form will be revealed as optimal

\begin{align*}
    s(t) = max\left(0, C(Pred(t-1 .. n)) \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

where $C(\mu(t-1), Pred(t-1))$ is given by the solution of the bellman equations. 

Consequently, I believe the following simpler strategy will achieve performance close to the bound.

\begin{align*}
    s(t) = max\left(0, C \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}
NOTE: In a finite MDP model, this is the strategy that one should take in the last round, regardless of the value of $\mu(t-1), Pred(t-1)$.

\textcolor{red}{Not done: Applying on traces} We can take a cellular trace and work backwards from $\mu(t)$ to get $Pred(t-1)$ (probabilistically pick a value of $Pred(t-1)$) given a $X^p$ (think of $X^p$ as evaluating a prediction strategy). We can then generate the performance bound and show how the above strategy performs on the trace.


\textbf{Model 3: Causal congestion control protocols, uncertainty in every time step can be different and is governed by a markov process.}

\begin{align*}
    \mu(t) &= \mu(t-1) \cdot X^{S(t-1)}
\end{align*}
Where $S(t)$ is the underlying markov variable. We prove the performance bounds for this model. 

\textcolor{red}{Not done: Posing it as a MDP} Posing the problem as a MDP and using bellman equations. For long run times, I believe this will reveal a strategy of the form

\begin{align*}
    s(t) = max\left(0, C_1(S(t-1)) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

where $C_1(S(t-1))$ is calculated using the Bellman equations. I also hypothesize the strategy 

\begin{align*}
    s(t) = max\left(0, C_2(S(t-1)) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

where $C_2(S(t-1))$ is calculated using insights from the lower bound (I can explain how $C_2$ is calculated) will be close to the predicted lower bound.

NOTE: Another way of thinking about this is that in a finite MDP model, this is the strategy that one should take in the last round.

\textcolor{red}{Not done: Applying on traces} Take a celllular trace assuming $S(t) = \mu(t)$ calculate different $X^{S(t-1)}$, and run the above strategy and see close are we get to the lower bound. 


\subsection{Why are these results useful?}
\begin{enumerate}
    \item This provides a way for CC researchers to analyze their control loops and see how close can they get to the optimal. A CC protocol might have additional components to deal with fairness, denoising observations, etc. They might be employing simple heuristics. It's a way for them to evaluate how close they are to the optimal and when should they stop iterating on the CC.
    \item Similarly CC researchers in the past have tried applying prediction techniques, the analysis can be useful for them to evaluate their prediction strategy.
    \item The optimal strategy requires an accurate value of the link capacity in the last time step, this implies e2e protocols which cannot infer past link capacity can perform sub-optimally.
    \item The optimal strategy also says that the queuing delay penalty term should be fixed. If you want to achieve a different tradeoff between utilization and queuing delay adjust the target utilization term (which can even go beyond 1). 
    \item The analysis for a generic markov model reveals the form of the control loop. Even if the hidden variables are unknown, it gives us a way to develop a reinforcement learning type model.
    \item Given the recent popularity of real time applications, the analysis reveals the performance an application can achieve on WiFi or cellular networks.
    \item The analysis reveals the uncertainty in link capacity is the culprit in bad performance. The analysis can be used to design schedulers (\eg cellular base stations) that bounds the uncertainity in link capacity to achieve better end-to-end performance.
    \item Researchers can build upon these methods to go a step further and evaluate even more complicated models.
    \item The same analysis can be applied to datacenter settings with per-flow scheduling to see what kind of performance can flows really achieve. It can be used to show on higher capacity links the performance degrades. (Meh)
\end{enumerate}
\fi

==> SIGMETRICS/miscellaneous.tex <==
\section{Miscellaneous}
\pg{Should we include any of these?}








\subsection{Analysis for metrics expressed not in expectation?}
What if we want to calculate 99th percentile queuing delay? Maybe given a (optimal) control loop, we can construct a Dicrete time markov chain model to analyse various statistics of the control loop.

\subsection{\pg{Personal Notes:}}
\begin{enumerate}
    \item What about multiple senders with different base RTTs?
    \item Implication of the strategy of form $r(t) = max(C_r, \frac{q(t-1)}{T})$. Spell it out why this strategy is the optimal in easy terms. Key idea is that in a given round the value function is only dependent on the value of r(t). This implies if $q(t-1)/T < optimal (r(t))$ then the best strategy is $r(t) = optimal r(t)$ regardless of $q(t-1)$. The interesting thing is the convexity of value function, which implies the best strategy is $r(t) = max(C_r, \frac{q(t-1)}{T})$. The value of $c_r$ might be dependent on the actual model of the link. In \S\ref{ss:generic_markov}, the value of $C_r$ is dependent on $S(t-1)$. A good guess for $C_r$ in this case can be the strategy given by conditions in theorem 3.4.
    \item Leveraging the fact that the strategy of the form above is the best strategy to construct an ML based algorithm that tries to figure out $C_r$ given the data. End-to-end vs explicit.
    \item note that the result in Theorem is general as long as the original function we are trying to minimize is convex, e.g, calculate L(t).
    \item Discussion, Related Work, Introduction, Abstract, title, background/motivation, limitation?
    \item stability analysis, continuous time vs discreet time, other metrics results, datacenter (uncertainity in competing flows), multiple flows, case for congestion control, how to use the control loop actually, multiple bottlenecks
\end{enumerate}



\if 0
\subsection{Calculating lost throughput instead of underutilization}

The extension above (\S\ref{s:model3}) can also be used to calculate the expected lost throughput and queuing delay trade-off. Assuming the link capacity variation model in \S\ref{s:model1}, let $L(t)$ be the lost throughput in round $t$. Then,

\begin{align}
     L(t) &= \frac{(\mu(t) \cdot T - s(t) \cdot T - Q(t - 1))}{T}^+\nonumber\\
     E[L(t)|\mu(t-1),r(t)=b] &= \mu(t-1) \cdot \int_{b}^{\infty}\left( a - b\right) \cdot f(a) \cdot da 
\end{align}

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{SIGMETRICS/images/miscellaneous/lost_throughput.pdf}
    \vspace{-4mm}
    \caption{\small Throughput lost vs. queueing delay.}
    \label{fig:lost_tput}
    \vspace{-4.5mm}
 \end{figure}

So even though the transition probabilities for link-rate are I.I.D, the performance bound (for $E[L(t)]$ and $E[q(t)]$) in a single round is dependent on $\mu(t-1)$ (the link state $S(t-1)$ in this case). We apply Model 3 to obtain a simplified strategy. \Fig{lost_tput} shows the performance for Model 1 ideal strategy and Model 3 style simplified strategy on the Verizon Uplink trace. We find that for different trade-off points on the model3 performance curve, the strategy uses a lower value of $C(\mu(t-1)$ for a lower value of $\mu(t-1)$. This is expected as when the link capacity ($\mu(t-1)$) is low, choosing a lower $C(\mu(t-1))$ will increase the lost throughput marginally while decreasing queuing delay more. 
\fi


==> conjecture.tex <==
\subsection{Proof of Conjecture:}
\label{ss:conjecture}
We will now prove the above conjecture by modelling the system as a Markov Decision Process (MDP), where the goal is to pick a sending rate strategy to minimize $w \cdot E[\frac{\bar{q}(t)}{T}] + E[\bar{U}(t)]$. \ma{Start by defining the MDP, and I think it would be better to drop the $1/T$ in the definition of the objective and value functions}  We will now write the Bellman Equation governing this optimization problem, for a finite number of rounds $n$. Where $V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1))$ \ma{why do you need the superscript 1?} is the value function at time step $t-1$
\begin{align}
    V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1)) &= \min_{s(t) \geq 0} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    &+ \int_{0}^{\infty}f(a) \cdot V_{t}^1(\frac{q(t)}{T},\mu(t)) \cdot da\Bigg)\nonumber &, \forall t\leqn\\
   V_{t}^1(\frac{q(t)}{T},\mu(t)) &= 0 & t=n\nonumber\\
    V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1)) &= min(\sum_{t=t}^{n}\Bigg(w \cdot E[\frac{{q}(t)}{T}] + E[{U}(t)]\Bigg))
\end{align}

The condition $s(t)\geq 0$ is equivalent to $r(t)\geq\frac{q(t-1)}{T}$. The equations can then be rewritten as,
\begin{align}
    V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1)) &= \min_{r(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    &+ \int_{0}^{\infty}f(a) \cdot V_{t}^1(\frac{q(t)}{T}, \mu(t)) \cdot da\Bigg)\nonumber &, \forall t\leq n\nonumber\\
     %V_{t-1}^1(\frac{q(t-1)}{T},\mu(t-1)) &= \min_{r(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
\end{align}

In the equation above, the first two terms on the right hand side depend only on the value of $r(t)$ and $q(t-1)$, as the random variables $U(t)$ and $q(t)$ are only dependent on $r(t)$. \ma{what if the 3rd term depends on $\mu(t-1)$? i think you can use induction to make this statement rigorous. } As a result, for describing the function $V_{t-1}^1$ we only need $q(t-1)$. Rewriting equations,  

\begin{align}
    V_{t-1}^1(\frac{q(t-1)}{T}) &= \min_{r(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    &+ \int_{0}^{\infty}f(a) \cdot V_{t}^1((\frac{r(t)}{a} - 1)^+) \cdot da\Bigg)\nonumber &, \forall t \leq n\nonumber\\
    % V_{t-1}^1(\frac{q(t-1)}{T}) &= \min_{r(t) \geq \frac{q(t-1)}{T}} \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)]\Bigg) &, t=n
\end{align}

\begin{theorem}
For all t, $V_{t-1}^1$ is convex.
\end{theorem}
We will give an induction proof for this.
\begin{lemma}
For all t, if  $V_{t}^1$ is convex, then, $V_{t-1}^1$ is convex.
\label{lemma:bellman_induction}
\end{lemma}

To prove this lemma, we will first prove three other lemmas. We define a new value function  $V_{t}^2(r(t))$ as follows,
\begin{align}
    V_{t-1}^1(\frac{q(t-1)}{T}) &= \min_{r(t) \geq \frac{q(t-1)}{T}} (V_{t}^2(r(t)))\nonumber\\
    %V_{t}^2(r(t)) &= \Bigg( w \cdot E[\frac{q(t)}{T}] + E[U(t)] \nonumber\\ 
    %&+ \int_{0}^{\infty}f(a) \cdot V_{t-1}^1((\frac{r(t)}{a} - 1)^+) \cdot da\Bigg)\nonumber &, \forall t<n\nonumber\\
\end{align}



\begin{lemma}
For all t, if $V_{t}^2$ is convex then $V_{t-1}^1$ is convex.
\end{lemma}
To prove this lemma we will show 
\begin{align}
    V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &\leq \alpha \cdot V_{t-1}^1(x) + (1 - \alpha) V_{t-1}^1(y)\nonumber\\
    & \forall \alpha \in [0,1], x,y\in\mathbb{R}^+, x<y
\end{align}

Let's assume that minima of $V_{t}^2$ occurs at $r(t)=C$ (need not be unique). Since $V_{t}^2$ is convex, 
\begin{align}
V_{t}^2(x)&\geq V_{t}^2(C) &x\geq C\nonumber\\
\Rightarrow   V_{t-1}^1(x) &= V_{t}^2(x) &\nonumber\\
V_{t}^2(x)&\leq V_{t}^2(C) &x< C\nonumber\\
\Rightarrow   V_{t-1}^1(x) &= V_{t}^2(C) &
\end{align}

Lets define a new function $h(x)$,
\begin{align}
    h(x) &=x & x \geq C\nonumber\\
    h(x) &= C & x < C\nonumber\\
     \Rightarrow V_{t-1}^1(x) &= V_{t}^2(h(x))
\end{align}
Note that $h(x)$ is convex.

\begin{align}
    V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &= V_{t}^2(h(\alpha \cdot x + (1 - \alpha) \cdot y)) \nonumber\\
    h(\alpha \cdot x + (1 - \alpha) \cdot y) &\leq \alpha \cdot h(x) + (1-\alpha) \cdot h(y)
\end{align}

Since, $h(x) \geq C, \forall x \in \mathbb{R}^+$,
\begin{align}
    V_{t}^2(h(\alpha \cdot x + (1 - \alpha) \cdot y)) &\leq V_{t}^2(\alpha \cdot h(x) + (1-\alpha) \cdot h(y))\nonumber\\
    \Rightarrow V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &\leq V_{t}^2(\alpha \cdot h(x) + (1-\alpha) \cdot h(y))\nonumber\\
    &\leq \alpha \cdot V_{t}^2(h(x)) + (1-\alpha) \cdot V_{t}^2(h(y))\nonumber\\
    &= \alpha \cdot V_{t-1}^1(x) + (1-\alpha) \cdot V_{t-1}^1(y)
\end{align}
\if 0
\textit{Case 1:} $\alpha \cdot x + (1-\alpha) \cdot y \leq C$,
\begin{align}
    V_{t-1}^1(x) &= V_{t}^2(C) \nonumber\\
    V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &= V_{t}^2(C) \nonumber\\
    V_{t-1}^1(y) &\geq V_{t-1}^1(x)\nonumber\\
                 &\geq V_{t}^2(C) \nonumber\\
    \Rightarrow V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &= \alpha \cdot V_{t}^2(C) + (1 - \alpha) V_{t}^2(C)\nonumber\\
    &= \alpha \cdot V_{t-1}^1(x) + (1 - \alpha) V_{t}^2(C)\nonumber\\
    & \leq \alpha \cdot V_{t-1}^1(x) + (1 - \alpha) V_{t-1}^1(y)
\end{align}
\textit{Case2:} $x\geq C$,
\begin{align}
    V_{t-1}^1(x) &= V_{t}^2(x)  \nonumber\\
    V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &= V_{t}^2(\alpha \cdot x + (1 - \alpha) \cdot y) \nonumber\\
    V_{t-1}^1(y) &= V_{t}^2(y) 
\end{align}
Since $V_t^2$ is convex,
\begin{align}
    V_{t}^2(\alpha \cdot x + (1 - \alpha) \cdot y) &\leq \alpha \cdot V_{t}^2(x) + (1-\alpha) \cdot V_{t}^2(y) \nonumber\\
    V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &\leq \alpha \cdot V_{t-1}^1(x) + (1 - \alpha) V_{t-1}^1(y)
\end{align}
\textit{Case 3:} $x \leq C \leq \alpha \cdot x + (1-\alpha) \cdot y$,
\begin{align}
    V_{t-1}^1(x) &= V_{t}^2(C)  \nonumber\\
    V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot y) &= 
    V_{t}^2(\alpha \cdot x + (1 - \alpha) \cdot y) \nonumber\\
    V_{t-1}^1(y) &= V_{t}^2(y) \nonumber\\
    \alpha \cdot x + (1 - \alpha) \cdot y &\leq \alpha \cdot C + (1 - \alpha) \cdot y\nonumber\\
    \Rightarrow V_{t-1}^1(\alpha \cdot x + (1 - \alpha) \cdot) y &\leq V_{t-1}^1(\alpha \cdot C + (1 - \alpha) \cdot y)\nonumber\\
    V_{t-1}^1(\alpha \cdot C + (1 - \alpha) \cdot y) &= V_{t}^2(\alpha \cdot C + (1 - \alpha) \cdot y)\nonumber\\
    &\leq \alpha \cdot V_{t}^2(C) + (1-\alpha) \cdot V_{t}^2(y) \nonumber\\
    &\leq \alpha \cdot V_{t-1}^1(x) + (1 - \alpha) V_{t-1}^1(y)
\end{align}
\fi 
Lemma proved.

\begin{lemma}
For all t, $V_{t-1}^1$ is non-decreasing, i.e., if $x \leq y$, $V_{t-1}^1(x) \leq V_{t-1}^1(y)$.
\end{lemma}
Lets assume that for $V_{t-1}^1(y)$ minima occurs at $r(t)=C_y$. Since, $C_y\geq y$, then, $C_y\geq x$. Thus, for $V_{t-1}^1(x)$ we can always pick $r(t)=C_y$, and, $V_{t-1}^1(x)$ is upper bounded by $V_{t-1}^1(y)$. Lemma proved.

\begin{lemma}
For all $t$, if $V_1^t$ is convex, then $V_2^t$ is convex.
\end{lemma}

\begin{align}
    V_{t}^2(x) &= ( w \cdot E[\frac{q(t)}{T}|r(t)=x] + E[U(t)|r(t)=x]) \nonumber\\ 
    &+ \int_{0}^{\infty}f(a) \cdot V_{t}^1((\frac{x}{a} - 1)^+) \cdot da\nonumber &, \forall t<n\nonumber\\
\end{align}

Lets define $h_a(x)$ as follows,
\begin{align}
    h_a(x) = (\frac{x}{a}-1)^+
\end{align}
The functions $h_a$ are all convex. Rewriting,
\begin{align}
    V_{t}^2(x) &= ( w \cdot E[\frac{q(t)}{T}|r(t)=x] + E[U(t)|r(t)=x]) \nonumber\\ 
    &+ \int_{0}^{\infty}f(a) \cdot V_{t}^1(h_a(x)) \cdot da\nonumber &, \forall t<n\nonumber\\
\end{align}
Since $h_a$ is convex, and $V_{t}^1$ in convex and non-decreasing, $V_{t}^1 \circ h_a$ is convex. Since summation of convex functions is convex, $V_{t}^2$ is convex. Lemma proved.

The last three lemmas, prove Lemma. ~\ref{lemma:bellman_induction}. Since $V_n^1$ is convex, by induction, theorem proved. %Conjecture proved.
The theorem establishes that the best strategy in a round $t$ is of the form $s(t) = max\left(0, C \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)$. \pg{TODO: To show that the best strategy in every round is the same we need to show that the value function in every round is the same.}

\pg{With the conjecture strategy we get a convex feasible set.}

==> extensions.tex <==
\section{Extensions}
\subsection{Incorporating Prediction}
The above math naturally works for link model of the following form,
\begin{equation}
    \mu(t) = Pred(t - 1) \cdot X_t
\end{equation}
where $Pred(t-1)$ is the prediction for the next round $t$, $X_i$ is an I.I.D random variable with $f$ as its probability density function (PDF). $X$ represents the deviation of the link rate from the predicted value. The equations can be rewritten as follows 

\begin{align}
    q(t) &= T \cdot \left(\frac{\frac{Q(t-1)}{T} + s(t)}{Pred(t - 1) \cdot X_t} - 1 \right)^+ \nonumber\\
    U(t) &= \left( 1 - \frac{\frac{Q(t-1)}{T} + s(t)}{Pred(t - 1) \cdot X_t}\right)^+\nonumber\\
    r(t) &=  \frac{\frac{Q(t-1)}{T} + s(t)}{Pred(t - 1)}  
\end{align}

With this model the trade-off can be calculated using only the distribution $f$. The condition for picking a fixed $r(t) = C_r$ in each round to achieve the lower bound (\S\ref{ss:tradeoff:lower_bound}) changes to 
\begin{align}
    Q(t) &\leq T \cdot C_r \cdot Pred(t) \nonumber\\
    C_r \cdot Pred(t-1) - Pred(t-1) \cdot X_{t} &\leq C_r \cdot Pred(t) \nonumber\\
    C_r \cdot Pred(t-1) - Pred(t-1) \cdot X_{min} &\leq C_r \cdot Pred(t)
\end{align}

\tom{is there a version of figure 7 that you could put here?  That is, use ML to predict the next rate from the previous rates, with no restrictions on the model, and pick some fixed $C_r$.  Overfitting is an issue so only do the training on the first half of the trace, and only report results on the second half. Does this outperform the previously optimal line based on an assumption of unpredictability in the subsequent rate?  Or would that graph look exactly the same as Figure 7?}

\subsection{Variable link rate transition}
So till now we assumed that the link rate transitions are same in every round. In this extension we assume there is some link state $I(t-1) \in \textbf{I}$, that governs the change in link rate from round $t - 1$ to $t$. The link state changes every round, but is independent of the queuing delay and sending rate. We assume that there is a steady distribution of probabilities over the link state. \tom{you mean steady state? you need some restriction on the probability distributions that the queue distribution is stable.}

\begin{align}
    \mu(t) = \mu(t-1) \cdot X^{I(t-1)}
\end{align}
where $X^{I(t-1)}$ is a random variable with PDF $f^{I(t-1)}$.

\pg{This model is a generic Markov Model for variations in the link capacity.} Since the PDF is dependent on the link state, we will get different trade-off curve for each round depending on the state in the previous round. \tom{As an example, the cellular link may have a maximum capacity, or that bandwidths tend to be mean-reverting. Are those handled by 2.1? or by 2.2?} Let $x, g^{I(t-1)}(x)$ represent a point on the trade-off curve in round t given $I(t-1)$, (note here the function $g^{I(t-1)}$ represents the queuing delay-underutilization trade-off frontier in round $t$ and is calculated using the method in \S\ref{ss:tradeoff:roundt} and is convex).

The question we now ask is what is the final trade-off boundary between under-utilization and queuing delay (given by curve $g$). Let $h(i)$ be the steady probability that $P(I(t-1) = i)$ for $t \to \infty$. The points in the feasible region of the new curve will be given by weighted average (using $h$) of points in the feasible region of curves $g^i$ where $i \in \textbf{I}$.  So curve $g$ is the boundary of points formed by taking points on the boundary of curves $g_i$. Let $\cup_{i \in \textbf{I}}(x^i, g^i(x^i))$ be the set of such points, then the final trade-off point ($(x,y)$) can be given by
\begin{align}
    x &= \sum_{i \in \textbf{I}} h(i) \cdot x^i\nonumber\\
    y &= \sum_{i \in \textbf{I}} h(i) \cdot g^i(x^i)
\end{align}

The point is considered on boundary if there is no other point $(x, y^1)$ such that $y^1 < y$. The condition for $(x,y)$ to be on the boundary ($y = g(x)$) is 
\begin{align}
    g^j '(x^j) &= g^k '(x^k) & \forall j,k \in \textbf{I}
\end{align}
i.e., by combining points with the same slope. To see why, consider that this is not the case for two states  $j, k$. Lets assume $g^j '(x^j) < g^k '(x^k)$, we can pick a new point $(x^1, y^1)$ corresponding to points $\cup_{i \in \textbf{I} - \{j,k\}} (x^i, g^i(x^i)) \cup (x^j + \frac{\epsilon}{h(j)}, g^j(x^j + \frac{\epsilon}{h^j})) \cup (x^k - \frac{\epsilon}{h(k)}, g^k(x^k - \frac{\epsilon}{h^k})$. If $\epsilon \to 0$, then the final trade-off point $(x^1, y^1)$ will be
\begin{align}
    x^1 &= \left(\sum_{i \in \textbf{I}}h(i) \cdot x^i\right) + h(j) \cdot \frac{\epsilon}{h(j)} - h(k) \cdot \frac{\epsilon}{h(k)} \nonumber\\
       &= x \nonumber\\
    y^1 &= \left(\sum_{i \in \textbf{I}}h(i) \cdot g^i(x^i)\right) + h(j) \cdot \frac{\epsilon}{h(j)} \cdot g^j '(x^j) - h(k) \cdot \frac{\epsilon}{h(k)} \cdot g^k '(x^k)\nonumber\\
     &= y + \epsilon \cdot (g^j '(x^j) - g^k '(x^k))
\end{align}
Since $x^1 = x$ and $y^1 < y$, the point $(x,y)$ cannot be on the boundary.

So by picking points on the trade-off curves $(x^i,g^i(x^i)$ with same slopes we can get different trade-off points $(x,y)$. The points $(x^i,g^i(x^i)$ will correspond to a fixed optimal strategy $r(t) = C_r^{I(t-1)}$. Note that with this model it is possible that $C_r^{I(t-1)} \neq C_r^{I(t)}$, as a result ABC (which closely emulates a fixed $r(t) = C_r$ regardless on the link state) will be sub-optimal. This can aid us in designing better congestion control schemes where we know a bit more about the system.

\textit{Final trade-off curve ($g$) is convex:}
Consider a point $(x,g(x))$ formed by combining $\cup_{i \in \textbf{I}}(x^i, g^i(x^i))$. Since $g^j'(x^j) = g^k'(x^k)$, $g'(x) = g^i'(x^i), \forall i \in \textbf{I}$. 

Consider another point $(x_1, g(x_1))$ formed by points $\cup_{i \in \textbf{I}}(x_1^i, g^i(x_1^i))$. If $g'(x) < g'(x_1)$, then $x < x_1$.
This is because
\begin{align}
    g'(x) &< g'(x_1) \nonumber\\
    g^i '(x^i) &< g^i '(x_1^i) & \forall i \in \textbf{I}
\end{align}
Since all the $g^i$ curves are convex with increasing slopes.
\begin{align}
    g^i '(x^i) &< g^i '(x_1^i) & \forall i \in \textbf{I} \nonumber\\
    x^i &< x_1^i & \forall i \in \textbf{I} \nonumber\\
    \sum_{i \in \textbf{I}} h(i) \cdot x^i &< \sum_{i \in \textbf{I}} h(i) \cdot x_1^i & \nonumber\\
    x &< x_1 & 
\end{align}
This implies that the curve $g$ is convex with increasing slope.

\textit{Conditions for achieving the lower bound on the trade-off:}
The question is can we follow the strategy $r(t) = C_r^{I(t-1)}$ such that the sending rate is non-negative.
\begin{align}
    Q(t) &\leq T \cdot C_r^{I(t)} \cdot \mu(t) & \forall I(t) \in \textbf{I}\nonumber\\
    (C_r^{I(t-1)} \cdot \mu(t-1) - \mu(t))^+ &\leq C_r^{I(t)} \cdot \mu(t) & \forall I(t-1), I(t) \in \textbf{I} \nonumber\\
    (\frac{C_r^{I(t-1)} }{X^{I(t-1)}} - 1)^+ &\leq C_r^{I(t)} & \forall I(t-1), I(t) \in \textbf{I} \nonumber\\
    \frac{C_r^{I(t-1)} }{X_{min}^{I(t-1)}} - 1) &\leq C_r^{I(t)} & \forall I(t-1), I(t) \in \textbf{I}
\end{align}

\textbf{Calculating lost throughput:}
The extension above can also be used to calculate the expected lost throughput and queuing delay trade-off. Assuming the link capacity variation model in \S\ref{s:tradeoff}, let $L(t)$ be the lost throughput in round $t$. Then,

\begin{align}
     L(t) &= \frac{(\mu(t) \cdot T - s(t) \cdot T - Q(t - 1))}{T}^+\nonumber\\
     E[L(t)|q(t-1), s(t),\mu(t-1)] &= \mu(t-1) \cdot \int_{r(t)}^{\infty}\left( x - r(t)\right) \cdot f(x) \cdot dx 
\end{align}

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/agg_tradeoff_Verizon_shortdown.pdf}
    \vspace{-4mm}
    \caption{\small Verizon Downlink. Throughput lost vs. queueing delay trade-off. The orange line shows the theoretical bound calculated using the description above. The blue line shows the curve calculated using a fixed $r(t) = C_r$ strategy in each round regardless on the link state $\mu(t-1)$.}
    \label{fig:lost_tput}
    \vspace{-4.5mm}
 \end{figure}

\pg{Note that all the individual trade-off curves for a given round are also convex. I proved it but am omitting it here.} So even though the transition probabilities for link-rate are I.I.D, the trade-off curve is dependent on $\mu(t-1)$ (the link state $I(t-1)$ in this case). We now calculate the trade-off for a Verizon cellular trace using the $f$ and $h$ calculated from the trace. \Fig{lost_tput} shows this bound. We find that for lower value of $\mu(t-1)$, the $C_r^{\mu(t-1)}$ is lower. This is expected as when the link rate ($\mu(t-1)$) is low, choosing a lower $C_r^{\mu(t-1)}$ will increase the lost throughput marginally while decreasing queuing delay substantially. 

\pg{I think for running this on a trace I need to calculate the $f^{\mu(t-1)}$ other wise the position of the curve is arbitrary compared to points from the real scheme.}

\pg{Personal ToDos:}
\begin{enumerate}
    \item What about multiple senders with different base RTTs?
    \item Double check the code for last part.
    \item Discuss the feasibility of such models. Try different traces. Also $r(t) = max(C_r, \frac{q(t)}{T})$ seems to build up a lot of queue with the model in \S\ref{s:tradeoff}.
    \item Try $f^{\mu(t-1)}$. Also calculate lost throughput in this case.
    \item Calculate the worse case scenario for a purely end to end scheme.
\end{enumerate}








==> extensions2.tex <==
\section{Extensions}
\label{s:extension}


\subsection{Markov Model for link capacity variation}
\label{ss:generic_markov}
The model in \S\ref{ss:simple_model} can be thought of as a markov process with the link capacity ($\mu(t)$) as the state and restrictions on the transition matrix. We will now generalize the model to a markov chain with very few restrictions. Let $\textbf{S}$ be the set of all possible states in the markov process, $S(t)$ denotes the  state in time step $t$. The state $S(t)$ in itself is a set, and includes the link capacity in that time step ($\mu(t)$). The state in round $t-1$ ($S(t-1)$) governs the state in time step $t$ ($S(t)$). $S(t-1)$ also implicitly governs the link capacity $\mu(t)$. The state $S(t)$ includes all other quantities that impact how the link capacity varies, e.g., in the cellular case, where multiple users are competing at a single base station, the number of users at the base station will be part of the state $S(t)$. In other words, this model takes into account all the quantities that can affect the link capacity under a markovian process. 

With this model we will establish a trade-off between $E[\bar{q}(t)]$ and $E[\bar{U}(t)]$ for causal congestion control protocols. Similar to model \S\ref{ss:simple_model}, the network consists of a single sender-receiver pair with a baseRTT $T$. Note that, the number of distinct states int the set $\textbf{S}$ can be infinite (i.e. continuous state space), for our proof we will assume the number of such states is finite (i.e. discrete state space). However, our argument holds for continuous state space as well. Let $\mathbb{A}$ be the transition matrix associated with the markov process. This matrix defines the probability $P^{A}(S(t)=k_1|S(t-1)=k_2)$. To calculate this trade-off, we will first convert this model to a from analogous to Equation. ~\ref{eq:simple_model_mu_def}. This markov model can be described in an alternate form given by the equations,
\begin{align}
    S(t)|(S(t-1)=k) &= Z_{t}^{k} \nonumber\\
    S(t) &= Z_{t}^{S(t-1)}
\end{align}
Where $\forall k \in \textbf{S}, Z_{t}^{k}$ is an I.I.D random variable. The PDF associated with these random variables $Z$ can be calculated using the original transition matrix $\mathbb{A}$. Since $\mu(t)$ is a given by $S(t)$, we can write $\mu(t)$ as follows,
\begin{align}
    \mu(t) &= Y_{t}^{S(t-1)}
\end{align}
Where $\forall k \in \textbf{S}, Y_{t}^{k}$ is an I.I.D random variable. Similarly, since $\mu(t-1)$ is given by $S(t-1)$, we can rewrite the above equation as follows,
\begin{align}
    \mu(t) &= \mu(t-1) \cdot X_{t}^{S(t-1)}
    \label{eq:generic_markov_mu_def}
\end{align}
Where $\forall k \in \textbf{S}, X_{t}^{k}$ is an I.I.D random variable. Let $f^s$ be the PDF associated with random variable $X^{k}$, $f^k$ can be calculated from the transition matrix $\mathbb{A}$. Notice the equation above has a very similar form to Equation. ~\ref{eq:simple_model_mu_def} from model \S\ref{ss:simple_model}.

\textit{Assumptions:} To establish the trade-off we assume the following. 1) The state transitions are independent of the decisions of the congestion control protocol itself, i.e., the sending rate and queuing delay do not affect how the state changes. 2) The markov model has a stationary distribution for the steady state given by the function $\pi$. $P(S(t)=k) = \pi(k), t \to \infty$. This implies that we cannot pick a arbitrary transition matrix, instead the transition matrix $A$ must meet the criterion (cite XXX) for stationary distribution in steady state. 3) The starting state ($S(0)$) has the same distribution as the stationary distribution $\pi$. This implies $P(S(t)=k) = \pi(k), \forall t \in \mathbb{N}$. 4) The link rate is always positive with the model, i.e., we only consider $A$ such that $P(\mu(t)<=0) = 0, \forall t \in \mathbb{N}$.


\begin{theorem}
In the model \S\ref{ss:generic_markov}, for any causal congestion control protocol, for any $t \in N$, there is a fundamental trade-off between $E[\bar{q}(t)]$ and $E[\bar{U}(t)]$. The point $\{E[\bar{q}(t)], E[\bar{U}(t)]\}$ lies in a convex set $\mathbb{D^A}$. The point $\{x,y\} \in \mathbb{D^A}$ iff
\begin{align}
    x = \sum_{k \in \textbf{S}} (\pi(k) \cdot x^k)\nonumber\\
    y = \sum_{k \in \textbf{S}} (\pi(k) \cdot y^k)
    \label{eq:thm:generic_markov}
\end{align}
where, $\forall k \in \textbf{S}$, the point $\{x^k, y^k\} \in \mathbb{C}^{f^k}$. The set $\mathbb{C}^{f^k}$ is as defined in Theorem. ~\ref{thm:simple_model_tradeoff} with $f^k$ as the PDF $f$. $f^k$ is the PDF of the random variable $X^k$, and is calculated using $\mathbb{A}$.
\label{thm:generic_markov}
\end{theorem}

The queuing delay and under-utilization in round $t$ is dependent on how link capacity changes from round $t-1$ to round $t$. We can calculate $E[q(t)]$ and $E[U(t)]$ using the conditional expected values $E[q(t)|S(t)=k]$ and $E[U(t)|S(t)=k]$ as follows
\begin{align}
    E[q(t)] &= E[E[q(t)|S(t)=k]]\nonumber\\
            &= \sum_{k \in \textbf{S}} (\pi(k) \cdot E[q(t)|S(t)=k])\nonumber\\
    E[U(t)] &= E[E[U(t)|S(t)=k]]\nonumber\\
            &= \sum_{k \in \textbf{S}} (\pi(k) \cdot E[U(t)|S(t)=k])
    \label{eq:generic_markov_equ}
\end{align}
To prove our theorem, we will prove the following lemma,
\begin{lemma}
 For any $k \in \textbf{S}$, the point $\{E[q(t)|S(t)=k],E[U(t)|S(t)=k]\} \in \mathbb{C}^{f^k}$.
\end{lemma}
The conditional queuing delay $(q(t)|(S(t)=k))$ and underutilization $(U(t)|S(t) = k)$ can be calculated as follows
\begin{align}
    q(t)|(S(t)=k) &= T \cdot \left(\frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1) \cdot X_{t}^{k}} - 1 \right)^+ \nonumber\\
                  &= T \cdot \left( \frac{r(t)}{X_{t}^k} -1 \right)^+\nonumber\\    
    U(t)|(S(t)=k) &= \left( 1 - \frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1) \cdot X_{t}^{k}}\right)^+\nonumber\\
                  &= \left(1 -  \frac{r(t)}{X_{t}^k} \right)^+     
    \label{eq:generic_markov_system}
\end{align}
Where $r(t)$ is as defined by Equation. ~\ref{eq:rt}. Notice that the equation above is analogous to Equation. ~\ref{eq:simple_model_qU_rt}. Thus, we can apply the same techniques as proof of Theorem. ~\ref{thm:simple_model_tradeoff}, the point $\{E[q(t)|S(t)=k], E[U(t)|S(t)=k]\}$ lies in the set $\mathbb{C}^{f^k}$, where $f^k$ is the PDF of the random variable $X^{k}$. Lemma proved.

The lemma above proves that $\forall t \in \mathbb{N}$, the point $\{E[q(t)], E[U(t)]\} \in \mathbb{D^A}$. The point $\{E[\bar{q}(t)], E[\bar{U}(t)]\}$ also belongs to $\mathbb{D^A}$ (using the same technique as the multi-round proof of Theorem ~\ref{thm:simple_model_tradeoff}). Theorem proved. 

\textbf{How to compute the set $\mathbb{D}^A$?}


To compute $\mathbb{D}^A$, we will first calculate the boundary function $g^A$. Point $\{x,y\}$ belongs to $\mathbb{D}^A$ iff $y \geq g^A$. The boundary point $\{x,g^A(x)\}$ must be a combination of points on the boundary of $\mathbb{C}^{f^k}$. More formally, 

\begin{align}
    x &= \sum_{k \in \textbf{S}} \pi(i) \cdot x^k\nonumber\\
    y &= \sum_{k \in \textbf{S}} \pi(i) \cdot g^{f^k}(x^k)
\end{align}
This is because for a given $x^k$, the min value of $y^k$, such that $\{x^k,y^k\} \in \mathbb{C}^{f^k}$ occurs at $y^k=g^{f^k}(x^k)$.

\begin{theorem}
The point $\{x,y\} \in \mathbb{D}^A$, given by 
\begin{align}
    x &= \sum_{k \in \textbf{S}} \pi(i) \cdot x^k\nonumber\\
    y &= \sum_{k \in \textbf{S}} \pi(i) \cdot g^{f^k}(x^k)\nonumber\\
\end{align}
is on the boundary or $y=g^A(x)$ iff
\begin{align}
    g^A'(x) = g^{f^k}'(x^k) &, \forall k \in \textbf{S}  
\end{align}
\end{theorem}

To prove this we will first show that if $y=g^A(x)$, then $g^{f^i}'(x^i) = g^{f^k}'(x^k), \forall i,j \in \textbf{S}$. We will prove this by contradiction. Lets assume, $g^{f^i} '(x^i) < g^{f^j} '(x^j)$. Then, we can pick a new point $(x_1, y_1)$ such that 
\begin{align}
    y_1^k &= g^{f^k}(x_1^k) &\forall k \in \textbf{S}\nonumber\\
    x_1^k &= x^k & \forall k \in \textbf{S} - \{i,j\}\nonumber\\
    \Rightarrow y_1^k &= g^{f^k}(x^k) &\forall k \in \textbf{S}-\{i,j\}\nonumber\\
    x_1^i &= x^i + \frac{\epsilon}{\pi(i)} &\nonumber\\
    \Rightarrow y_1^i &= y^i + \frac{\epsilon}{\pi(i)}g^{f^i}'(x^i) & \nonumber\\
    x_1^j &= x^j - \frac{\epsilon}{\pi(j)} &\nonumber\\
    \Rightarrow y_1^j &= \frac{\epsilon}{\pi(j)}g^{f^j}'(x^j) &
\end{align}

If $\epsilon \to 0$, then $\{x_1, y_1\}$ can be given by
\begin{align}
    x_1 &= \left(\sum_{k \in \textbf{S}}\pi(k) \cdot x^k\right) + \pi(i) \cdot \frac{\epsilon}{\pi(i)} - \pi(j) \cdot \frac{\epsilon}{\pi(j)} \nonumber\\
       &= x \nonumber\\
    y_1 &= \left(\sum_{k \in \textbf{S}}\pi(k) \cdot g^i(x^i)\right) + \pi(i) \cdot \frac{\epsilon}{\pi(i)} \cdot g^{f^i} '(x^i) - \pi(j) \cdot \frac{\epsilon}{\pi(j)} \cdot g^{f^j} '(x^j)\nonumber\\
     &= y + \epsilon \cdot (g^{f^i} '(x^i) - g^{f^j} '(x^j))
\end{align}
Since $x_1 = x$ and $y_1 < y$, the point $(x,y)$ cannot be on the boundary. Contradiction.

Finally, we will show that if the point $\{x,y\}$ satisfies the theorem conditions, then it will be on the boundary. To do this we will show that there does not exist another point $\{x_1,y_1\}$ which satisfies the theorem conditions and $x=x_1$ but $y_1<y$. Lets assume $g^{f^k}'(x^k) = C$ and $g^{f^k}'(x_1^k) = C_1$. Lets assume $C < C1$. Since $g^{f^k}$ in convex with increasing slope,
\begin{align}
    g^{f^k}'(x^k) &< g^{f^k}'(x_1^k) &\forall k \in \textbf{S}\nonumber\\
    \Rightarrow x^k &< x_1^k &\forall k \in \textbf{S}\nonumber\\
    \Rightarrow x &< x_1 &
\end{align}
Since $x<x_1$, we have a contradiction. We can show a similar contradiction if $C>C1$ (we will get $x>x_1$). For $C=C_1$, since $g^{f^k}$ is convex, if $x=x_1$, then $y=y_1$. This is because
\begin{align}
    y_1^k &= g^{f^k}(x_1^k) & k \in \textbf{S}\nonumber\\
          &= g^{f^k}(x^k + (x_1^k - x^k))& k \in \textbf{S}\nonumber\\
          &= g^{f^k}(x^k) + g^{f^k}' \cdot (x_1^k - x^k)& k \in \textbf{S}\nonumber\\
          &= g^{f^k}(x^k) + C \cdot (x_1^k - x^k)& k \in \textbf{S}\nonumber\\
    y_1 &= y + C \cdot \sum_{k \in \textbf{S}}(x_1^k - x^k) &\nonumber\\
    \Rightarrow y_1 &= y &
\end{align}
Theorem proved!

\if 0
\pg{marker to skip. Regarding the remainder of the proof/statements, I want to talk first before making further progress.}

The question we now ask is what is the final trade-off boundary between under-utilization and queuing delay (given by curve $g$). Let $h(i)$ be the steady probability that $P(I(t-1) = i)$ for $t \to \infty$. The points in the feasible region of the new curve will be given by weighted average (using $h$) of points in the feasible region of curves $g^i$ where $i \in \textbf{I}$.  So curve $g$ is the boundary of points formed by taking points on the boundary of curves $g_i$. Let $\cup_{i \in \textbf{I}}(x^i, g^i(x^i))$ be the set of such points, then the final trade-off point ($(x,y)$) can be given by
\begin{align}
    x &= \sum_{i \in \textbf{I}} h(i) \cdot x^i\nonumber\\
    y &= \sum_{i \in \textbf{I}} h(i) \cdot g^i(x^i)
\end{align}

The point is considered on boundary if there is no other point $(x, y^1)$ such that $y^1 < y$. The condition for $(x,y)$ to be on the boundary ($y = g(x)$) is 
\begin{align}
    g^j '(x^j) &= g^k '(x^k) & \forall j,k \in \textbf{I}
\end{align}
i.e., by combining points with the same slope. To see why, consider that this is not the case for two states  $j, k$. Lets assume $g^j '(x^j) < g^k '(x^k)$, we can pick a new point $(x^1, y^1)$ corresponding to points $\cup_{i \in \textbf{I} - \{j,k\}} (x^i, g^i(x^i)) \cup (x^j + \frac{\epsilon}{h(j)}, g^j(x^j + \frac{\epsilon}{h^j})) \cup (x^k - \frac{\epsilon}{h(k)}, g^k(x^k - \frac{\epsilon}{h^k})$. If $\epsilon \to 0$, then the final trade-off point $(x^1, y^1)$ will be
\begin{align}
    x^1 &= \left(\sum_{i \in \textbf{I}}h(i) \cdot x^i\right) + h(j) \cdot \frac{\epsilon}{h(j)} - h(k) \cdot \frac{\epsilon}{h(k)} \nonumber\\
       &= x \nonumber\\
    y^1 &= \left(\sum_{i \in \textbf{I}}h(i) \cdot g^i(x^i)\right) + h(j) \cdot \frac{\epsilon}{h(j)} \cdot g^j '(x^j) - h(k) \cdot \frac{\epsilon}{h(k)} \cdot g^k '(x^k)\nonumber\\
     &= y + \epsilon \cdot (g^j '(x^j) - g^k '(x^k))
\end{align}
Since $x^1 = x$ and $y^1 < y$, the point $(x,y)$ cannot be on the boundary.

So by picking points on the trade-off curves $(x^i,g^i(x^i)$ with same slopes we can get different trade-off points $(x,y)$. The points $(x^i,g^i(x^i)$ will correspond to a fixed optimal strategy $r(t) = C_r^{I(t-1)}$. Note that with this model it is possible that $C_r^{I(t-1)} \neq C_r^{I(t)}$, as a result ABC (which closely emulates a fixed $r(t) = C_r$ regardless on the link state) will be sub-optimal. This can aid us in designing better congestion control schemes where we know a bit more about the system.
\fi

\begin{corollary}
For model in \S~\ref{ss:generic_markov}, function $g^A$ is convex.
\end{corollary}
Consider a point $\{x_1,g^A(x_1))\}$ formed by combining $\cup_{k \in \textbf{S}}\{x_1^k, g^{f^k}(x_1^k)\}$. 

Consider another point $\{x_2, g^A(x_2)\}$ formed by points $\cup_{k \in \textbf{S}}\{x_2^k, g^{f^k}(x_2^k)\}$. To prove, $g^A$ is convex, we need to show if $g^A'(x_1) < g^A'(x_2)$, then $x_1 < x_2$.
\begin{align}
    g^A'(x_1) &< g^A'(x_2) \nonumber\\
    \Rightarrow g^{f^k} '(x_1^k) &< g^{f^k} '(x_2^k) & \forall k \in \textbf{S}
\end{align}
Since all the $g^{f^k}$ curves are convex with increasing slopes.
\begin{align}
    g^{f^{k}} '(x_k^i) &< g^{f^k} '(x_2^k) & \forall k \in \textbf{S} \nonumber\\
    \Rightarrow x_1^k &< x_2^k & \forall k \in \textbf{S} \nonumber\\
    \sum_{k \in \textbf{S}} \pi(k) \cdot x_1^k &< \sum_{k \in \textbf{S}} \pi(k) \cdot x_2^k & \nonumber\\
    x_1 &< x_2 & 
\end{align}
This implies that the curve $g^A$ is convex with increasing slope. This implies, the set $\mathbb{D}^A$ is convex.

\pg{SKIP}

\textit{Conditions for achieving the lower bound on the trade-off:}
The question is can we follow the strategy $r(t) = C_r^{I(t-1)}$ such that the sending rate is non-negative.
\begin{align}
    Q(t) &\leq T \cdot C_r^{I(t)} \cdot \mu(t) & \forall I(t) \in \textbf{I}\nonumber\\
    (C_r^{I(t-1)} \cdot \mu(t-1) - \mu(t))^+ &\leq C_r^{I(t)} \cdot \mu(t) & \forall I(t-1), I(t) \in \textbf{I} \nonumber\\
    (\frac{C_r^{I(t-1)} }{X^{I(t-1)}} - 1)^+ &\leq C_r^{I(t)} & \forall I(t-1), I(t) \in \textbf{I} \nonumber\\
    \frac{C_r^{I(t-1)} }{X_{min}^{I(t-1)}} - 1) &\leq C_r^{I(t)} & \forall I(t-1), I(t) \in \textbf{I}
\end{align}

\textbf{Calculating lost throughput:}
The extension above can also be used to calculate the expected lost throughput and queuing delay trade-off. Assuming the link capacity variation model in \S\ref{s:model1}, let $L(t)$ be the lost throughput in round $t$. Then,

\begin{align}
     L(t) &= \frac{(\mu(t) \cdot T - s(t) \cdot T - Q(t - 1))}{T}^+\nonumber\\
     E[L(t)|q(t-1), s(t),\mu(t-1)] &= \mu(t-1) \cdot \int_{r(t)}^{\infty}\left( x - r(t)\right) \cdot f(x) \cdot dx 
\end{align}

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/agg_tradeoff_Verizon_shortdown.pdf}
    \vspace{-4mm}
    \caption{\small Verizon Downlink. Throughput lost vs. queueing delay trade-off. The orange line shows the theoretical bound calculated using the description above. The blue line shows the curve calculated using a fixed $r(t) = C_r$ strategy in each round regardless on the link state $\mu(t-1)$.}
    \label{fig:lost_tput}
    \vspace{-4.5mm}
 \end{figure}

\pg{Note that all the individual trade-off curves for a given round are also convex. I proved it but am omitting it here.} So even though the transition probabilities for link-rate are I.I.D, the trade-off curve is dependent on $\mu(t-1)$ (the link state $I(t-1)$ in this case). We now calculate the trade-off for a Verizon cellular trace using the $f$ and $h$ calculated from the trace. \Fig{lost_tput} shows this bound. We find that for lower value of $\mu(t-1)$, the $C_r^{\mu(t-1)}$ is lower. This is expected as when the link rate ($\mu(t-1)$) is low, choosing a lower $C_r^{\mu(t-1)}$ will increase the lost throughput marginally while decreasing queuing delay substantially. 

\pg{I think for running this on a trace I need to calculate the $f^{\mu(t-1)}$ other wise the position of the curve is arbitrary compared to points from the real scheme.}

\pg{Personal Notes:}
\begin{enumerate}
    \item What about multiple senders with different base RTTs?
    \item Implication of the strategy of form $r(t) = max(C_r, \frac{q(t-1)}{T})$. Spell it out why this strategy is the optimal in easy terms. Key idea is that in a given round the value function is only dependent on the value of r(t). This implies if $q(t-1)/T < optimal (r(t))$ then the best strategy is $r(t) = optimal r(t)$ regardless of $q(t-1)$. The interesting thing is the convexity of value function, which implies the best strategy is $r(t) = max(C_r, \frac{q(t-1)}{T})$. The value of $c_r$ might be dependent on the actual model of the link. In \S\ref{ss:generic_markov}, the value of $C_r$ is dependent on $S(t-1)$. A good guess for $C_r$ in this case can be the strategy given by conditions in theorem 3.4.
    \item Leveraging the fact that the strategy of the form above is the best strategy to construct an ML based algorithm that tries to figure out $C_r$ given the data. End-to-end vs explicit.
    \item note that the result in Theorem is general as long as the original function we are trying to minimize is convex.
    \item Discuss the feasibility of such models. Try different traces. Also $r(t) = max(C_r, \frac{q(t-1)}{T})$ seems to build up a lot of queue with the model in \S\ref{s:model1}.
    \item For model in \S\ref{ss:generic_markov} prove the convexity property formally. The convexity of the value function is given a $S(t-1)$.
    \item Try $f^{S(t-1)}$. Also calculate lost throughput in this case.
\end{enumerate}








==> introduction.tex <==
\section{Introduction}
\label{s:intro}
Recently, there has been a surge in the new congestion control protocols proposed for time-varying wireless links such as Cellular or WiFi ~\cite{abc, sprout, verus, copa, pcc}. The goal of any such protocol is to reduce queue at the bottleneck link while maintaining a high utilization or throughput. Time-varying links exhibit variations in link capacity over time, achieving both low queuing and high utilization is challenging.

In this work, we establish the limits on performance of congestion protocols on time-varying links. We show there is a \textit{fundamental} trade-off between underutilization and queuing delay for any causal congestion control scheme where the sender picks the sending rate based on observations in the past (i.e., the sender is not predicting the link capacity in future).

Intuitively, the bound on trade-off is fundamental because the sender adjusts its rate based on observations such as queuing delay, link capacity, etc. in the past (delayed by the propagation delay). By the time sender adjusts its rate, the link conditions might have changed. The randomness of the change in link capacity can cause the sender to either under-utilize the link (if the link capacity increased) or build up excessive queuing. Note that this trade-off is not because the link capacity is changing but because the sender doesn't know how the link capacity is changing deterministically.


We begin by modelling the randomness on variations in link capacity using a discrete-time stochastic model. Under this model, the link capacity at a time step $t$ is a random variable dependent on the link capacity at time step $t-1$. In particular, the randomness in the link capacity in any given time step is similar. With this model, we prove a bound on the expected underutilization-expected queuing delay trade-off. Any causal congestion control protocol will achieve the same or worse trade-off than this bound. We also provide close to optimal congestion control strategies that either achieve the trade-off bound or are very close. The bound itself is a function of the randomness in capacity variations. On increasing the randomness, the bound worsens.  


We then expand this model to incorporate non-causal congestion control protocols with future predictions of link capacity, and show that the trade-off bound improves as the prediction gets better. We also expand our link variation model to a generic markov chain model.


\subsection{What results/theorems have we proved?}
We present analysis on performance of congestion control protocols on links with time-varying capacity. Because of the uncertainty in the link capacity, any protocol can only achieve a certain link utilization queuing delay trade-off. the The analysis reveals a bound on the performance a protocol can achieve and also reveals the optimal congestion control protocol. We model the link capacity ($\mu(t)$) as discrete time stochastic process. We consider three stochastic processes.

\textbf{Model 1: Causal congestion control protocols, uncertainty in link capacity is similar in each time step.}
\begin{align*}
    \mu(t) = \mu(t-1) \cdot X
\end{align*}
where $X$ is a random variable with PDF $f$. A key characteristic of this model is the uncertainty in link capacity in every time-step is similar (characterized by $f$). This assumption makes the model easy to analyze and provides a good starting point. We prove a lower bound on the performance in terms of expected queuing delay and link underutilization using stochastic analysis (see \S\ref{ss:model1:performance_bound}) for causal congestion control protocols. 

\textit{MDP.} To find the optimal congestion control strategy we pose the problem as a MDP with achieving high utilization and low queuing delay as the objective function. Using Bellman equations to describe the system, we can find the optimal strategy (see \S\ref{ss:conjecture}). Interestingly, we find that for infinitely long runtime, the optimal strategy is very simple

\begin{align*}
    s(t) = max\left(0, C \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

\textcolor{red}{Not done: Close the gap in the proof above.} We need to make this statement precise.

\textcolor{red}{Not done: Generalizing the MDP.} We can generalize the objective function in the MDP. I think the result holds as long as the objective function is just a function of $r(t)$ and is convex in $r(t)$.

\textit{Application to real traces.} We applied the model on a few cellular traces. The bound on performance on these traces seem real, existing congestion control schemes achieve performance worse than the predicted bound. We also ran the above optimal strategy and found the performance is actually very close to the predicted bound.

\textbf{Model 2: Predictive congestion control protocols,  uncertainty in link capacity is similar in each time step.}
\begin{align*}
    \mu(t) = Pred(t-1) \cdot X^p
\end{align*}
where $Pred(t-1)$ is the link capacity prediction for round $t$. This is a model which assumes that the protocol makes a prediction for the next round and the link capacity varies from the prediction in an uncertain way. The equations governing the system are very similar to the one in Model 1. We prove a bound on performance similar to model 1, depends only on $f^p$ (PDF of $X^p$), see \S\ref{s:model2}.  

\textcolor{red}{Not done: Posing it as a MDP} Posing the problem as a MDP and using bellman equations. I believe this will not reveal a simple optimal strategy as in Model 1. My guess is a strategy of the following form will be revealed as optimal

\begin{align*}
    s(t) = max\left(0, C(Pred(t-1 .. n)) \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

where $C(\mu(t-1), Pred(t-1))$ is given by the solution of the bellman equations. 

Consequently, I believe the following simpler strategy will achieve performance close to the bound.

\begin{align*}
    s(t) = max\left(0, C \cdot Pred(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}
NOTE: In a finite MDP model, this is the strategy that one should take in the last round, regardless of the value of $\mu(t-1), Pred(t-1)$.

\textcolor{red}{Not done: Applying on traces} We can take a cellular trace and work backwards from $\mu(t)$ to get $Pred(t-1)$ (probabilistically pick a value of $Pred(t-1)$) given a $X^p$ (think of $X^p$ as evaluating a prediction strategy). We can then generate the performance bound and show how the above strategy performs on the trace.


\textbf{Model 3: Causal congestion control protocols, uncertainty in every time step can be different and is governed by a markov process.}

\begin{align*}
    \mu(t) &= \mu(t-1) \cdot X^{S(t-1)}
\end{align*}
Where $S(t)$ is the underlying markov variable. We prove the performance bounds for this model. 

\textcolor{red}{Not done: Posing it as a MDP} Posing the problem as a MDP and using bellman equations. For long run times, I believe this will reveal a strategy of the form

\begin{align*}
    s(t) = max\left(0, C_1(S(t-1)) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

where $C_1(S(t-1))$ is calculated using the Bellman equations. I also hypothesize the strategy 

\begin{align*}
    s(t) = max\left(0, C_2(S(t-1)) \cdot \mu(t-1) - \frac{Q(t-1)}{T}\right)
\end{align*}

where $C_2(S(t-1))$ is calculated using insights from the lower bound (I can explain how $C_2$ is calculated) will be close to the predicted lower bound.

NOTE: Another way of thinking about this is that in a finite MDP model, this is the strategy that one should take in the last round.

\textcolor{red}{Not done: Applying on traces} Take a celllular trace assuming $S(t) = \mu(t)$ calculate different $X^{S(t-1)}$, and run the above strategy and see close are we get to the lower bound. 


\subsection{Why are these results useful?}
\begin{enumerate}
    \item This provides a way for CC researchers to analyze their control loops and see how close can they get to the optimal. A CC protocol might have additional components to deal with fairness, denoising observations, etc. They might be employing simple heuristics. It's a way for them to evaluate how close they are to the optimal and when should they stop iterating on the CC.
    \item Similarly CC researchers in the past have tried applying prediction techniques, the analysis can be useful for them to evaluate their prediction strategy.
    \item The optimal strategy requires an accurate value of the link capacity in the last time step, this implies e2e protocols which cannot infer past link capacity can perform sub-optimally.
    \item The optimal strategy also says that the queuing delay penalty term should be fixed. If you want to achieve a different tradeoff between utilization and queuing delay adjust the target utilization term (which can even go beyond 1). 
    \item The analysis for a generic markov model reveals the form of the control loop. Even if the hidden variables are unknown, it gives us a way to develop a reinforcement learning type model.
    \item Given the recent popularity of real time applications, the analysis reveals the performance an application can achieve on WiFi or cellular networks.
    \item The analysis reveals the uncertainty in link capacity is the culprit in bad performance. The analysis can be used to design schedulers (\eg cellular base stations) that bounds the uncertainity in link capacity to achieve better end-to-end performance.
    \item Researchers can build upon these methods to go a step further and evaluate even more complicated models.
    \item The same analysis can be applied to datacenter settings with per-flow scheduling to see what kind of performance can flows really achieve. It can be used to show on higher capacity links the performance degrades. (Meh)
\end{enumerate}


==> tradeoff.tex <==
\section{Underutilization-delay trade-off}
\label{s:tradeoff}
\subsection{Model}
We consider a network with a single sender and receiver pair connected via a time-varying link. We are considering a discrete time model, where each discrete round's duration is $T$, the base RTT for the sender-receiver pair. The capacity of the link in round t ($\mu(t)$) is given by the following rule
\begin{equation}
    \mu(t) = \mu(t - 1) \cdot X_t
\end{equation}
where $X_i$ is an I.I.D random variable with $f$ as its probability density function (PDF). \pg{We will show that in a particular time step $t$, the trade-off between under-utilization and delay is just a function of the variability in the link capacity in that time step(capture by the random variable $X$). We begin by evaluating/analyzing the situation where the variability in each time step (represented by the random variable $X$) is same. Under such a model we will prove that there are simple congestion control strategies that one can follow to achieve the best trade-off without knowing anything about the PDF $f$ of the random variable $X$. We will then use this initial model to analyze a extension of the model where the variability in link capacity in a time step is dependent on all the information available in the previous time steps (Markov Model).}

\tom{define that we are studying finite # of rounds. study Q (underutilization) as a function of s(t). Underutil in round t is equation 6. Queuing delay in round t is in equation 5 (warning maybe not - or at least, the notion of "delay" is a bit unclear here, because the service rate is variable - maybe easier to say overutilization, rather than queueing delay, as that's scaled to the round's rate).  consider only algorithms of the following type (e.g., has knowledge of queue and rate in previous round, chooses any sequence of s(t) >= 0, as an arbitrary function of everything you have seen up to time t-1, and the distribution f.  cannot depend on Xt : s(t) is a random variable, depends on values of u(0..t-1) and X(0..t-1).  s(t) must be measurable. Cannot be a function of anything that occurs from time t or later.) So what is the theorem: curve between underutil and queueing space, every algorithm in the class we study, will fall within feasible range (bounded by curve). Curve depends on distribution X.  You are not saying that by luck you could fall outside of the curve - on a particular sample path you can be lucky, but in expectation you cannot be.  and that the curve is convex, etc.}

\tom{some additional work: there exists feasible algorithms that are tight for some constrained versions of X, a specific algorithm, such as Cr is a constant. Claim this does well for most distributions. But are there worst case distributions that push it away from the bound?  e.g., high probability it is epsilon. low probability it is very high.}

With this model we want to capture link capacity variations of wireless links such as a cellular link for a user. The equation above can be rewritten as follows
\begin{align}
    ln(\mu(t)) &= ln(\mu(t - 1)) + ln(X_t)\nonumber\\ 
               &= ln(\mu(0)) + \sum_{i=1}^{t}ln(X_i)
\end{align}
Then,
\begin{align}
    E[ln(\mu(t))] &= E[ln(\mu(0) + \sum_{i=1}^{t}ln(X_i)]\nonumber\\ 
               &= ln(\mu(0)) + t \cdot E[ln(X)]
\end{align}
With the above link model, if we don't want the link rate to either drift positively or negatively over time, then 
\begin{equation}
    E[ln(X)] = 0
\end{equation}
\pg{Why did we use this instead of $E[X] = 1$ that would give $E[\mu(t)] = \mu(0)$? The reason is if you take a link capacity trace for a real network time varying link such that the start and end capacity are the same, and use it to fit the model above (i.e. calculate the PDF $f$); then, $E[ln(X)]$ will be equal to zero, however, its not necessary that $E[X]$ will be 1. Maybe the problem here is that real time-varying link traces don't follow the model above. With the above model the link capacity can get arbitrarily close to 0 or approach $\infty$.}
\ma{I don't think we should conflate the model with the trace stuff for now. The problem with E(logX) = 0 is that it implies that EX <= 1 (and EX < 1 unless X=1 with prob. 1). This means that $E(\mu(t)) \to 0$ as $t \to \infty$. We also need a requirement that P(X > 0) = 1?}
\tom{why we can't just say $E(X) = 1$ and $E(ln x) = 0$ - that is the expected value of the geometric series is 1.
- ok its an abstraction and a real physical link isn't quite like that,
but it is a simple model that would be easily understood, especially since you will fix it later with
the HMM. I'm not sure the rest of the math above is getting you anywhere. I think you would lose pretty much everyone if the
outcome of our analysis really depends, in step 1, that E(X)!=1 or E(ln X) != 0.}

Let s(t) be the sending rate, Q(t) be the queue size and q(t) be the queuing delay in round t. Then the system is described by the following equations. \tom{to be pedantic, q(t) is NOT the queueing delay in round t. It is the queue size scaled by the drain rate in round t. There is no guarantee that the drain rate is the same in subsequent rounds.}
\tom{At each step, provide intuition in English - its not that hard.  Something like: the queue in each round depends on the previous queue, plus the difference between the estimated and actual link bandwidth.  We then normalize by the actual link bandwidth, to provide a scaled estimate of the over utilization of the link in round t.} \pg{I agree, in time varying settings $q(t)$ is not queuing delay. I should have added this note earlier. Regarding intuition, maybe I am being lazy, but I want to get the math verified first and then talk about how to write this paper properly.}

\begin{align}
    Q(t) &= (Q(t-1) + s(t) \cdot T- \mu(t) \cdot T)^+\nonumber\\
    q(t) &= \frac{Q(t)}{\mu(t)}\nonumber\\
         &= \frac{(Q(t-1) + s(t) \cdot T - \mu(t) \cdot T)^+}{\mu(t)}\nonumber\\
         &= T \cdot \left(\frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t)} - 1 \right)^+\nonumber\\
         &= T \cdot \left(\frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1) \cdot X_t} - 1 \right)^+
    \label{eq:queue_dynamics}
\end{align}

where $y+ = max(0, y)$.


Similarly, let U(t) be the underutilization in round t, then,

\begin{align}
    U(t) &= \frac{(\mu(t) \cdot T - s(t) \cdot T - Q(t - 1))^+}{\mu(t) \cdot T}\nonumber\\
         &= \left( 1 - \frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1) \cdot X_t}\right)^+
    \label{eq:undeutilization_dynamics}
\end{align}

\subsection{Trade-off}
\label{ss:tradeoff:roundt}
Now we will establish a fundamental bound on the trade-off between underutilization and queuing delay. Let's define a new variable $r(t)$ as a function of $Q(t-1)$ and $s(t)$.
\begin{align}
  r(t) =  \frac{\frac{Q(t-1)}{T} + s(t)}{\mu(t - 1)}  
\label{eq:rt}
\end{align}


Note that we defined this new variable only for ease of mathematical manipulation. \tom{I don't believe that qualifier is needed, or accurate.} \pg{I don't know about needed, but I think I defined it mostly for ease of following the math later.} Intuitively, $r(t)$ can be thought of as an indicator of load on the link in round $t$ \tom{scaled by the expected value of the capacity, given the capacity in round t-1, that is, the load in round t-1.  But if we change the expected value (e.g., with more information), don't you want to be able to rescale the mean?} \pg{No, it is not dependent on the mean. Rather the scaling is dependent on the $state$ in the link model $\mu(t) = state \cdot X$. Note than in the link model described in Sec 2.2 it is not necessary that the random variable $X$ will have an expectation of 0.}. Then rewriting Eq. ~\ref{eq:queue_dynamics} and ~\ref{eq:undeutilization_dynamics} we get,
\begin{align}
    q(t) &= T \cdot \left(\frac{r(t)}{X_t} - 1 \right)^+\nonumber\\
    U(t) &= \left(1 - \frac{r(t)}{X_t}\right)^+
\end{align}
The expected value in round t can then by given by
\tom{i'm not sure what it means for the expectd value to be conditional on those other values, and only those values.  r(t) depends on u(t-1) too.  otoh, since you want to say that they only depend on r(t), and r(t) depends on q(t-1) and s(t) and $\mu(t-1)$, isn't that enough?}\pg{Yes we can just say it depends on $r(t)$. But the trade-off curve in itself is independent of anything.}
\begin{align}
    E[q(t)|q(t-1),s(t)] &= E[T \cdot \left(\frac{r(t)}{X_t} - 1 \right)^+]\nonumber\\
                        &= T \cdot \int_{0}^{r(t)}\left(\frac{r(t)}{x} - 1 \right) \cdot f(x) \cdot dx\\
    E[U(t)|q(t-1), s(t)] &= E[\left( 1 - \frac{r(t)}{X_t}\right)^+]\nonumber\\
                         &= \int_{r(t)}^{\infty}\left( 1 - \frac{r(t)}{x}\right) \cdot f(x) \cdot dx 
\end{align}
Note that the expected value of both $U(t)$ and $q(t)$ only depends on $r(t)$. \tom{as we would expect, increasing the rate we send, in an uncertain environment, poses a direct tradeoff between under and overutilization} Increasing $r(t)$ increasing expected value of $q(t)$ buunder andt reduces the expected value of $U(t)$ . Varying $r(t)$ we will get a trade-off curve.
 

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/roundt_uniform.pdf}
    \vspace{-4mm}
    \caption{\small Trade-off in a given round t. $X \sim \textit{U}(0.27, 2) $, $T = 0.1$s.}
    \label{fig:roundt_uniform}
    \vspace{-4.5mm}
 \end{figure}
 \Fig{roundt_uniform} shows this trade-off when $X$ is derived from a uniform distribution. Note that regardless of $r(t)$, the expected values of queuing delay and underutilization will lie precisely on the curve. See that this curve is convex in shape. We will now formally prove this \tom{avoid antecedents at critical points} and use it to establish the trade-off over multiple rounds.
 
\tom{move to appendix - I realize convexity is important but only the math nerds will doubt it. At the very least, you need to say something like, convex independent of the pdf of the random walk as the result here, since it seems hard to imagine how it would not be true.}
 
\textit{Trade-off curve in round t is convex:}
Using Leibniz integral rule,
\begin{align}
    \frac{d(E[q(t)|q(t-1),s(t)])}{dr(t)} &= T \cdot \frac{d\left(\int_{0}^{r(t)}\left(\frac{r(t)}{x} - 1 \right) \cdot f(x) \cdot dx\right)}{dr(t)}\nonumber\\
    %\frac{E[q(t)|q(t-1),s(t)]}{dr(t)} &= T \cdot \frac{d \left(r(t)\int_{0}^{r(t)}\frac{f(x)}{x} \cdot dx \right)}{dr(t)} - T \cdot \frac{d \left(\int_{0}^{r(t)}f(x) \cdot dx \right)}{dr(t)}\nonumber\\
    %\frac{E[q(t)|q(t-1),s(t)]}{dr(t)} &= T \cdot \frac{d \left(r(t)\int_{0}^{r(t)}\frac{f(x)}{x} \cdot dx \right)}{dr(t)} - T \cdot f(r(t))\nonumber\\
    %\frac{E[q(t)|q(t-1),s(t)]}{dr(t)} &= T \cdot \left(\int_{0}^{r(t)}\frac{f(x)}{x} \cdot dx \right) + T \cdot \left(r(t) \cdot \frac {f(r(t)}{r(t)}\right) - T \cdot f(r(t))\nonumber\\
                                        &= T \cdot \left(\int_{0}^{r(t)}\frac{f(x)}{x} \cdot dx \right)
\end{align} 
Similarly,
\begin{align}
    \frac{d(E[U(t)|q(t-1),s(t)])}{dr(t)} &= \frac{d\left(\int_{r(t)}^{\infty}\left(1 -\frac{r(t)}{x}\right) \cdot f(x) \cdot dx\right)}{dr(t)}\nonumber\\
                                         &= -\int_{r(t)}^{\infty}\frac{f(x)}{x
    } \cdot dx
\end{align}
Combining the equations above we get
\begin{align}
    \frac{d(E[U(t)|q(t-1),s(t)])}{d(E[q(t)|q(t-1),s(t)])} &= - \frac{\int_{r(t)}^{\infty}\frac{f(x)}{x
    } \cdot dx}{T \cdot \left(\int_{0}^{r(t)}\frac{f(x)}{x} \cdot dx \right)}
\end{align}
Note that in the above equation the denominator is increasing with $r(t)$ while the absolute value of numerator is decreasing, this implies that as we increase $r(t)$ (and consequently $E[q(t)|q(t-1),s(t)]$) the absolute slope of the trade-off graph in round t is decreasing.  Therefore, the curve is convex irrespective of the PDF $f$.

\textbf{Trade-off over multiple rounds:}
\tom{isn't the size of a range the absolute value of the range? $|t_{range}|$ - seems notationally easier than including sum of 1; or maybe even simpler is saying "average".}
We will now calculate \tom{generalize the result to compute} the lower bound of the trade-off over multiple rounds ($t_{range}$) between $E[\bar{q}(t_{range})|r(t_{range})]$ and  $E[\bar{U}(t_{range}|r(t_{range})]$, where $\bar{q}(t_{range}) = \frac{\sum_{t \in t_{range}} q(t)}{\sum_{t \in t_{range}} 1}$, and $\bar{U}(t_{range}) = \frac{\sum_{t \in t_{range}} U(t)}{\sum_{t \in t_{range}} 1}$.

\begin{align}
    E[\bar{q}(t_{range})|r(t_{range})] &= \frac{\sum_{t \in t_{range}}{E[q(t)|r(t)]}}{\sum_{t \in t_{range}} 1}\nonumber\\
    E[\bar{U}(t_{range})|r(t_{range})] &= \frac{\sum_{t \in t_{range}}{E[U(t)|r(t)]}}{\sum_{t \in t_{range}} 1}
\end{align}

\tom{i must admit I did not follow this explanation. I think your goal is to justify that for the multiround case, r(t) is a constant, but I'm not sure - because you say it is about explaining the tradeoff, but then you launch into assuming $C_{R}$ in the next section, even though that term is never defined and introduced only in the middle of the paragraph.  You should start with the goal (whatever it is), and then explain how the steps are required for that goal.}
Given a value of $r(t_{range})$, we can get expected values of $\bar{q}$ and $\bar{U}$. To get the final trade-off point we can take a average of the trade-off point in each round corresponding to $r(t), t \in t_{range}$. For different values of $r(t_{range})$, we will get different final trade-off points. The final trade-off region is the region spanned by final trade-off points corresponding to all the values of $r(t_{range})$. Since the trade-off curve for a single round is convex, and that trade-off curve in each round is same, the boundary of the trade-off for multiple rounds will be the same as trade-off curve in a single round. In particular, the final trade-off point will be on the boundary if and only if $r(t) = C_r, \forall t \in t_{range})$ where $C_r$ is a positive constant. \pg{Note that this statement is true assuming a smooth curve for the trade-off in a given round and the slope of the curve is changing (i.e. the slope is not constant).}

By varying $C_r$ we vary the final trade-off point. For other values of of $r(t_{range})$, the expected value of $\bar{q}$ and $\bar{U}$ will lie in the space within this boundary. The boundary of the final curve represents the fundamental limit on the trade-off between underutilization and queuing delay that any congestion control scheme cannot surpass \tom{given the assumptions of the link model}. Put in other words regardless of the sending rate strategy (that will give a $r(t_{range}$), one cannot achieve a better trade-off under \tom{for?} this link model. \tom{since you haven't shown that the model holds in any useful sense for a real link, I'd soft peddle the "hey we're optimal" part here. You are optimal for a model you constructed, not too surprisingly.}

\tom{If all you are concerned about is a mechanism for estimating a time varying link, then you will do the obvious thing and pick a point on the curve.  that doesn't seem hard or conceptually deep. But we have a number of existing CC mechanisms, however, and we can ask how well they do? All must be feasible given the link model, but we can see whether they approach optimal in this case or lie away from it for some reason.}

\begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/feasible_uniform.pdf}
    \vspace{-4mm}
    \caption{\small Trade-off over multiple rounds. $X \sim \textit{U}(0.27, 2) $, $T = 0.1$s. The grey region presents that feasible region of any congestion control protocol.}
    \label{fig:feasible_uniform}
    \vspace{-4.5mm}
 \end{figure}
 
 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/f_variation.pdf}
    \vspace{-4mm}
    \caption{\small Trade-off is dependent on PDF $f$.}
    \label{fig:f_variation}
    \vspace{-4.5mm}
 \end{figure}
 
 \Fig{feasible_uniform} shows this trade-off bound and the feasible region. This trade-off is fundamentally dependent on the PDF $f$. \Fig{f_variation} shows the bound for two uniform distributions, as the range of $f$ decreases the trade-off gets better.
 
 \subsection{When is the trade-off lower bound achievable?}
 \label{ss:tradeoff:lower_bound}
 The points on the trade-off boundary correspond to $r(t) = C_r, \forall t \in t_{range}$. From Eq. ~\ref{eq:rt}, it implies that the sending rate $s(t)$ must be equal to $C_r \cdot \mu(t-1) - \frac{Q(t-1)}{T}, \forall t \in t_{range}$ for us to be on the boundary. If the $Q(t-1)$ become high ($> T \cdot C_r \cdot \mu(t-1)$, because of say variations in the link capacity), then $s(t)$ will have to be negative, which is not possible. \tom{not obvious that this follows! You derived that Cr is constant under an assumption that s(t) could be negative.  So its not clear that there is still a Cr if s(t) cannot be negative.  If we constrain s(t) to non-negative values, leaving Cr constant, then in any round, r(t) > Cr.}\pg{I have not assumed anything. I am simply saying the point on the trade-off boundary corresponds to $r(t) = C_r$ in every round. Then the question I am asking is a sending rate policy that gives you $r(t) =C_r$ possible? The answer depends on the $C_r$ you are choosing and the bounds on variation in the link model itself.} As a result, $r(t) > C_r$, and the trade-off point will be inside the boundaries.
 
\tom{more explanation needed here too.  You are deriving constraints on the PDF f, such that the above solution holds (i think). You need to say that.  And I'm not sure, retrospectively, if it wouldn't be better for you to simply say, early on, that we constrain f in such as a way as the solution is feasible.  The form of that constraint is derived here.  But doesn't the constraint on f depend in a very direct way on our choice of Cr?  And so Cr isn't really a constant?  That is, if we find ourselves falling behind, might we decide to change Cr before we become unfeasible?} We will now establish under what condition is the boundary point corresponding to a given $C_r$ is achievable. Let $X_{min}$ be the minimum value of $X$ given the PDF $f$ ($P(X<X_{min}) = 0$). Lets assume that $Q(t - 1) 
 \leq T \cdot C_r \cdot \mu(t-1)$, then we can pick a not negative $s(t)$, such that $r(t) = C_r$. Then in the next round $t$,
 \begin{align}
     Q(t) &= (Q(t-1) + s(t) \cdot T- \mu(t) \cdot T)^+\nonumber\\
          &= (T \cdot C_r \cdot \mu(t - 1) - T \cdot \mu(t))^+\nonumber\\
          &=  T \cdot \mu(t) \cdot (\frac{C_r}{X_t} - 1)^+
 \end{align}
 In order to be able to pick a non-negative sending rate $s(t+1)$ in the next round such that $r(t+1) = C_r$, 
 \begin{align}
    Q(t) &\leq T \cdot C_r \cdot \mu(t) \nonumber\\
    (\frac{C_r}{X_t} - 1)^+ &\leq C_r \nonumber\\
    \frac{C_r}{X_t} - 1 &\leq C_r \nonumber\\
    {C_r}(\frac{1}{X_t} - 1) &\leq 1 \nonumber\\
    C_r &\leq \frac{1}{\frac{1}{X_{min}} - 1}
\label{eq:boundary_condition} 
 \end{align}
 So the bound is achievable if and only if the above condition is met. For explicit congestion control schemes that know $q(t-1)$ and $\mu(t-1)$ in round $t$, if the above condition is met, then they can always pick a $s(t)$ such that $r(t)=C_r, \forall t \in t_{range}$ and the bound is achievable. \pg{For $C_r$ for which the above condition is not met, we conjecture the following strategy, $r(t) = max(C_r, \frac{Q(t)}{T \cdot \mu(t-1)})$ or $s(t) = (\mu(t-1) \cdot C_r - \frac{Q(t-1)}{T})^+$ will be optimal.}
 
 \tom{I think you need something more here. The point you are making, I think, is that if you can bound the deviation
 per round, then there is a feasible portion of the curve with r=constant, and the tighter that bound, the more of the curve that is available to you.  E.g. with Xmin of .5, the only part of the curve you can use is the upper half.
 But you aren't saying, I think, there is no way to solve the problem if you want the tradeoff to be in the "infeasible"
 portion.  It is just that your derivation does not say what should happen in that case.  Now I don't think the solution
 will turn out to be all that different in that case - its just you don't have a proof for it. For example, could you allow an effective value of negative s by borrowing from the future?}
 
  \begin{figure}
 \centering
    \begin{subfigure}[tbh]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/tradeoff_Verizon_shortdown.pdf}
         \vspace{-7mm}
        \caption{Trade-off}
        \label{fig:verizon_down:trade-off}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.36\textwidth}
        \includegraphics[width=\textwidth]{images/pdf_Verizon_shortdown.pdf}
        \vspace{-7mm}
        \caption{PDF}
        \label{fig:verizon_down:pdf}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Verizon Downlink}
    \label{fig:verizon_down}
    \vspace{-4mm}
\end{figure}

 \begin{figure}
 \centering
    \begin{subfigure}[tbh]{0.4\textwidth}
        \includegraphics[width=\textwidth]{images/tradeoff_Verizon_shortup.pdf}
         \vspace{-7mm}
        \caption{Trade-off}
        \label{fig:verizon_up:trade-off}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.36\textwidth}
        \includegraphics[width=\textwidth]{images/pdf_Verizon_shortup.pdf}
        \vspace{-7mm}
        \caption{PDF}
        \label{fig:verizon_up:pdf}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small Verizon Uplink}
    \label{fig:verizon_up}
    \vspace{-4mm}
\end{figure}

\subsection{Applying the model to Cellular traces:}
\Fig{verizon_down} and \Fig{verizon_up} shows the trade-off for two Verizon cellular traces. To generate the trade-off we empirically calculated the PDF $f$ from the trace. The figures also show performance of a number of schemes on these traces in an emulation (using Mahimahi). ABC is an explicit scheme that comes closest to the frontier. \tom{one sentence description of ABC's rule needed here.} In fact, the ABC sender's rate closely corresponds to $r(t) = 0.98$ in each round. The ABC point lies close to $C_r = 0.98$ point. Note that, the condition in Eq. ~\ref{eq:boundary_condition} is not met with $C_r = 0.98$, however in both the trace probability $X < \frac{1}{\frac{1}{C_r} + 1}$ or $X < 0.5$is fairly low, as a result excessive queue buildup that hinders the ability to pick a fixed $r(t) = C_r$ is rare.

The other congestion control schemes in the figure are purely end-to-end, and as a result the sender might not know $\mu(t-1)$ in round $t$ if the link was underutilized in round $t-1$. As a result, these schemes \textit{will} be unable to pick a sending rate corresponding to a $r(t) = C_r$ in such rounds, and the trade-off will thus deviate from the boundary.

 \begin{figure}[t]
     \centering
    \includegraphics[width=0.8\columnwidth]{images/tradeoff_Verizon_shortup_abc_eta.pdf}
    \vspace{-4mm}
    \caption{\small Verizon Uplink. Performance of ABC with different value of $\eta$. abc\_tcp\_x implies ABC with x/100 as $\eta$. With $\eta = x$, ABC is very similar to a policy $r(t) = C_r = x$.}
    \label{fig:verizon_up_eta}
    \vspace{-4.5mm}
 \end{figure}
 
 \Fig{verizon_up_eta} shows performance of ABC with different values of $\eta$. With different value of $\eta$m ABC achieves a different throughput queuing delay trade-off. All the points sit very close to the boundary.
